Optimal Control with $L^\infty$ and Integral Cost Functionals

Many control problems are classically formulated using integral costs that capture the cumulative performance of a system. Peak or worst-case behavior is captured via supremum or $L^\infty$-costs in another variety of control problems. When both cumulative and peak performance are important, it is natural to consider objective functions that combine the two costs. Although each criterion is well studied, their combination has not been explored extensively and we precisely work on such control problems. Towards establishing the existence, we first consider the relaxed framework, where control is considered using probability distributions. Using the well-known compactness and convexity properties of such control spaces, we establish the existence of an optimal relaxed control---we eventually establish the existence of an $\epsilon$-optimal pure (or classical) control, for every $\epsilon > 0.$ Despite these existence results, computing optimal policies remains challenging due to the non-smoothness introduced by the supremum term, and it is not clear whether the dynamic programming principle holds for our combined problem. To address this, we introduce a family of smooth approximations that yield standard control problems with well-defined optimal (pure) solutions. Using Maximum Theorem, we establish that the solutions of the smooth problems among pure controls form $\epsilon$-optimal for the original problem, with $\epsilon$ tending to zero as the smoothing parameter converges to zero. Finally using the methods proposed in this paper, we study a queueing problem to illustrate (among others) that the required trade-off between peak congestion levels and cumulative performance can be achieved.

==> app.tex <==

\appendix 
\setcounter{section}{1}
%%\renewcommand{\thesection}{\Roman{section}}

\section{ Brief summary of results from \cite{warga2014optimal}}
\label{app_sec}

We will re-produce important notations, definitions and entities of  book \cite{warga2014optimal}   in our own notations and according to our requirements. 




\subsection{Relaxed controls and Lemma \ref{lemma_space_compact}} 
\label{App_relaxed_control}
We begin with  some definitions of \cite[Section IV, pg. 263]{warga2014optimal}.
We adopt standard notations commonly used in the optimal control community, which differ from those in \cite{warga2014optimal}. To facilitate cross-referencing, we summarize the mapping between both the sets of symbols in Table \ref{Table_notations}.


Let  $C(U)$ be the space of continuous functions from $U$ to  real line $\mathbb{R}$, 
$L^1(T, C(U))$ be the space of integrable functions from $T$ to $C(U)$  (see $m_\g$ defined in Definition \ref{defn_relaxed_weak_conv}),
$$
\g \in L^1(T, C(U)), \mbox{ iff } \int_0^{t_1} \sup_{u \in U} |g(t, u)|   dt = \int_0^{t_1}   m_\g(t)   dt < \infty.
$$
Let
$L^1(T, C(U))^\star$ be its topological dual  (see Table \ref{Table_notations} for corresponding notations in \cite{warga2014optimal}).  

For any $\X$ a normed linear separable space, let $|.|_w$ represent the weak norm on its dual $\X^\star$,
\begin{equation}
 |f|_w := \sum_{i} 2^{-i} \frac{ |f(x_i)| }{1+ |f(x_i)|},   \mbox{ for all } f \in \X^\star, 
 \label{Eqn_weak_norm_fw}
\end{equation}
defined using a countable dense set $\{x_1, x_2, \cdots, \}$ of $\X$ (by well known Banach-Alaoglu theorem \cite{rudin1991functional}, unit ball in $\X^\star$ is compact under the corresponding weak-topology).  Let frm($U$)  be the vector space of   Radon measures on set $U$ and  rpm$(U) = \P(U)$ be  the set of   Radon probability measures on $U$. It is well known (Riesz
representation theorem \cite{warga2014optimal}) that  frm($U$) is  the dual of space of continuous functions, i.e.,   frm$(U) =C(U)^\star$---one can thus equip frm($U$) with weak-norm using the dense subset of $C(U)$, as in \eqref{Eqn_weak_norm_fw} and then the space of probability measures rpm$(U)$ is its subset.
 

Let  
$\N$ be the set of  $\muL$   or Lebesgue measurable functions   ${\mathbf \nu} : T \to (\mbox{frm}(U), |.|_w) $ such that $\mbox{ess sup}     |\nu(t)| (U)   < \infty$, where $\mbox{ess sup}$ is wrt $\muL$ measure. By \cite[Theorem  IV.1.8, pp 268]{warga2014optimal}, $\N$ is isomorphic\footnote{Each $\nu \in \N$, defines one  linear functional ${\mathdutchbcal l}_\nu $  on   $ L^1(T, C(U))$:
$$
{\mathdutchbcal l}_\nu(g):= \int_0^{t_1}\muL(dt) \int_U g(t, u) \nu(t, du)  \mbox{ for all } g \in L^1(T, C(U)),  \mbox{ is  a  linear functional}.
$$The mapping $\nu \mapsto {\mathdutchbcal l}_\nu$ is an isomorphism from $\N$ to  
$(L^1(T, C(U) ) )^\star$ (\cite{warga2014optimal}).
} to the topological dual, $L^1(T, C(U))^\star$. Thus one can also equip $\N$ with weak-norm as in \eqref{Eqn_weak_norm_fw}, since   
$L^1(T, C(U))$ is also separable, see also \cite[Section IV.1]{warga2014optimal}. Further, $\N$ is metrizable \cite[Subsection VI.1.9]{warga2014optimal}. 

Next the space of relaxed controls is defined as the following subset of $\N$, whose range is the space of probability measures (recall rpm$(U) = \P(U)$, see \cite[Page 263]{warga2014optimal}) 
\begin{eqnarray}
  \hspace{13mm}  \Sscr &=& \{ \nu \in \N : \nu (t) \in \mbox{rpm}(U), \mbox{ for almost all } t \in T  \} 
    \label{Eqn_calS_defn_app}\\
    && \hspace{-10mm} = \  \{ \bsig :T \to \P(U), \mbox{ which is measurable}\},  \mbox{ which equals that defined in \eqref{eqn_calS_defn}}.  \nonumber
\end{eqnarray}
    

The next set of   definitions are from \cite[Section IV.3, pg. 279]{warga2014optimal}. In our case, the set of restrictions $U^\hash (t) = U $, the entire control space, for all $t$, as we don't have any restrictions (in \cite{warga2014optimal}, this is referred to as $R^\hash(t)$). 
Thus the space of relaxed controls, $\Sscr$ in \eqref{eqn_calS_defn} or \eqref{Eqn_calS_defn_app}, coincides with   $\Sscr^\hash = \Sscr$ of 
\cite{warga2014optimal}.
As a result Lemma \ref{lemma_space_compact}
is true using the results of chapter~IV. Furthermore, $\Sscr$ is a subset of metrizable space $\N$ and hence is metrizable. \eop 

 

\begin{table}[h]
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
      & Notations of \cite{warga2014optimal} & This paper & Remarks \\ \hline
1    & $R$  & $  U$    &     Compact control space         \\ \hline
2   & $C(R)$ & $C(U)$ &     Space of continuous functions on $U$  \\ \hline
3  & $L^1(T, C(R))$ & $L^1(T, C(U))$  &     Space of $\muL$ integrable functions on $C(U)$  \\ \hline
4         & frm   $(S)$ &     frm   $(U)$ &  Space of Radon measures     on  $U$             \\ \hline
5     &  rpm   $(S) $   &     rpm   $(U) = \P(U)$   &   Space of Radon probability measures     on  $U$             \\ \hline
6       &   $\Sscr $  &   $\Sscr$ &   Space of  relaxed controls             \\ \hline 
7       &   $\R$ &    $\U(T)$  &   Space of  original (or pure) controls             \\ \hline 
\end{tabular}
\vspace{2mm}
\caption{ Notations of this paper and that in \cite{warga2014optimal}}
\label{Table_notations}
\end{table}


\newcommand{\Z}{{\cal Z}}
\newcommand{\yy}{{\bf y}}


\subsection{Relaxed trajectories and proof of Theorem \ref{thm:relaxed_controls_refined}} 
\label{App_relaxed_trajectories}

\textbf{Proof of part (a).}
Consider  the solution of $\bdot{ z} = K_f (1+{z})$, with $z(0) = |x_0|$,  for $K_f$ given in the uniform-boundedness assumption \ref{assum_a1},  which  equals  $z_{x_0}(t) =(1+|x_0|)e^{K_f t} -1 $,  for any $t \in T$, $x_0 \in \I$ (here $| \cdot |$ also represents the Euclidean norm). 
Now  
 observe, using the standard results in ODE literature (see \cite[Chapter 1]{piccinini2012ordinary}), the 
 ODE \eqref{Eqn_relaxed_dynamics_refined} has  \textit{unique} solution  $\x_{\bsig, x_0}$, 
 for any relaxed control $\bsig\in \Sscr$, under  assumption \ref{assum_a1},  which   can be upper bounded:  
 $$
 |x_{\bsig, x_0}(t)| \le z_{x_0}(t), \mbox{ for all   } t\in T, \ x_0 \in \I.
 $$ 
 
Define the following terms,  all of which are finite by assumptions \ref{assum_a0}-\ref{assum_a1} and after domination by $z_{x_0}$ trajectories---here  $T, U$, $\I$  are compact and $f$ is    continuous:
\begin{equation}
 \zeta(t) := \max_{ |x| \le z_{x_0}(t), \  u \in U,   x_0 \in \I }  | f(t, x, u) | \mbox{  for each } t \in T \mbox{ and, } \overline{\zeta} := \max_{t\in T} \zeta(t) .
\label{Eqn_bar_psi}
\end{equation}
Using the above bounds, we have the following:  
\begin{eqnarray}
\label{Eqn_f_upperbounds}
  \hspace{10mm}  | f(t, x_{\bsig, x_0}(t), u) | &\le  & \overline{\zeta}, \quad  \mbox{ for all } t \in T, \mbox{ $\bsig \in \Sscr$, $u\in U$ and $x_0 \in \I$, } \mbox{ and } \\
 \hspace{10mm}   
  \max_{t, \bsig, x_0} |x_{\bsig, x_0} (t) |  &\le  & \bar z := \max_{t \in T, x_0 \in \I} |z_{x_0}(t) | , \mbox{ for all $\bsig \in \Sscr$ and $x_0 \in \I$.}  \label{Eqn_upperbounds}
\end{eqnarray}
%Further define $\overline{\psi} := \sup_{t\in T} \psi(t) .$ 
Now consider the following `projected  set'  of  only relaxed trajectories, see \eqref{Eqn_A_set}:
$$
\T := \{ \x : 
 (\x, \bsig, x_0) \in \A, \mbox{ for some } \bsig \in \Sscr, x_0 \in \I \}  \subset C(T).
 $$
 By \eqref{Eqn_upperbounds}, the above collection is bounded (point-wise also). 
Further, using the bound of \eqref{Eqn_f_upperbounds}, 
for any $\x \in \T$, there exists some $(\bsig,x_0)$  such that $(\x, \bsig, x_0) \in \A$ (in other words, $\x= \x_{\bsig, x_0}$), and then we have the following integral form and boundedness:
\begin{eqnarray}
\hspace{5mm}
   \left | x (\tau_2) - x(\tau_1) \right  |=  \left |\int_{\tau_1}^{\tau_2} f(s, x(s), \sigma(s)) ds \right |  \le    {\overline{\zeta}} (\tau_2-\tau_1), \mbox{ for all } 0 \le \tau_1 \le \tau_2 \le t_1, 
\end{eqnarray}
implying the collection in $\T$ are equicontinuous. 
Thus by  Arzelà--Ascoli theorem (see, \cite{warga2014optimal}), $\T $ is relatively compact   under uniform topology, given by $\|\cdot \|_\infty$. Therefore, \textit{its closure $cl(\T)$ is compact and  sequentially compact}.


\textbf{Proof of $\T$ is closed and compact under uniform topology:}
Let $\{\x_n\} \subset \T$ be a sequence such that 
$\|\x_n - \x\|_\infty \to 0$, or converges uniformly on $T$.
By definition of $\T$ and ODE \eqref{Eqn_relaxed_dynamics_refined}, for each $n$,  there exist $\bsig_n \in \Sscr$ and $x_{0n} \in \I$ such that 
\begin{equation}
x_n(t) = x_{0n} + \int_0^t f(s,x_n(s),\sigma_n(s))\,ds,  \mbox{ for all } t \in T.
\label{Eqn_xn}
\end{equation}

Since $\I$ is compact, there exists a subsequence (for simplicity of notations, relabel with original indices) such that
$x_{0n} \to  x_0 \in \I.$
By Lemma \ref{lemma_space_compact},  $\Sscr$ is sequentially compact under the relaxed-weak topology, thus there exists a further subsequence (again after relabeling) such that
$\bsig_n \rwc  \bsig \in \Sscr$ and 
$x_{0n} \to  x_0 \in \I.$

Taking limits as $n \to \infty$ for the integral term in the right hand side of \eqref{Eqn_xn}, we have the following convergence by the Dominated Convergence Theorem (wrt $\muL$ measure),
\begin{eqnarray}
\label{Eqn_integral_ctns}
\int_0^t f(s,x_n(s),\sigma_n(s))\,ds
\to
\int_0^t f(s,x(s),\sigma(s))\,ds \mbox{ for all } t \in T, 
\end{eqnarray}
because   each  such $[0, t] \subset T $ and as, 
\begin{itemize}
\item  $x_n (s) \to x (s)$, for all $s \in T$, by  uniform convergence  on $T$, given  by hypothesis;
\item $\sigma_n  (s) \to \sigma 
(s)$ for all $s \in T$, by convergence in relaxed-weak topology,
\item  thus  
$f(s,x_n(s),\sigma_n(s)) \to f(s,x(s), \sigma(s))$
for all $s \in T$, 
   by continuity of $f$; 
\item  $|f(s,x_n(s),\sigma_n(s))| \le \overline{\zeta}$, for all $s \in T$ (dominated by integrable, actually a constant function). 
\end{itemize}
Considering limit $n\to \infty$ for both sides of \eqref{Eqn_xn}, we finally have that:  for each $t \in T$, 
$
x(t) =  x_0 + \int_0^t f(s,x(s), \sigma(s))\,ds,
$
which shows that $\x = \x_{\bsig,x_0}$ and thus  $\x \in \T$. 
Therefore     $\T$ is closed  and thus $\T = cl(\T)$  is compact in the uniform  topology.  

\textbf{Proof of $\A$ is Compact.} Observe that
$\A \subsetneq \T \times \Sscr \times \I.$
Since $\T$, $\Sscr$, and $\I$ are compact, their product is compact under the product topology. 
Suffices to prove $\A$ is closed, towards that consider a sequence 
$(\x_n,\bsig_n,x_{0n}) \in \A, \mbox{ such that } (\x_n,\bsig_n,x_{0n}) \to (\x,\bsig,x_0)$. 
Then, using  the same arguments as before, we obtain
\begin{equation}
    x(t) = x_0 + \int_0^t f(s,x(s),\sigma(s))\,ds, \mbox{ for all } t \in T,
    \label{Eqn_x_integral_form}
\end{equation}
and thus that $\x = \x_{\bsig,x_0}$, equals the solution under $(\bsig, x_0)$---hence $(\x, \bsig, x_0) \in \A$. Therefore,  $\A$ is closed  and so is compact. This completes the proof of part (a). 

\textbf{Proof of part (b)---Continuity of the ODE solution.} 
We obtain this proof using the parametric continuity provided by the Maximum theorem (see \cite{berge1877topological}) and we begin with some definitions.  Consider the following  parameterized function   $\Upsilon: \T \times \Sscr \times \I \to [0, \infty)$, defined as below, with $(\bsig, x_0) \in \Sscr\times \I$ as parameters: 
\begin{eqnarray} \hspace{10mm}
  \Upsilon (\x; \bsig, x_0 ) :=  \int_0^{t_1} \left ( x(t) -  x_0 - \int_0^t f(s, x(s), \sigma(s) ) ds \right )^2   dt, \quad  \mbox{ for all }  \x \in \T. 
    \label{Eqn_gamma_max_thm}
\end{eqnarray}
Now recall     $\x_{\bsig, x_0}$ is the unique solution of ODE \eqref{Eqn_relaxed_dynamics_refined}, for any given  $(\bsig, x_0)$---at such an $\x = \x_{\bsig, x_0}$, the integrand in \eqref{Eqn_gamma_max_thm} is zero for all $t \in [0, t_1]$ because of the integral representation of the ODE solution (see \eqref{Eqn_x_integral_form})---thus
the   function in \eqref{Eqn_gamma_max_thm}  possesses a unique minimizer in the form of the relaxed trajectory  $\x_{\bsig, x_0}$  for any $(\bsig, x_0)$---and this is because:
$$
\min_{\x \in \T } \Upsilon (\x; \bsig, x_0 ) = \Upsilon (\x_{\bsig, x_0}; \bsig, x_0) = 0, \ \  \mbox{also observe  by construction, }  \Upsilon (\x; \bsig, x_0) \ge 0. 
$$

Thus we have unique minimizer for  the  function in \eqref{Eqn_gamma_max_thm} and 
$$
a_\Upsilon^*(\bsig, x_0) := \mbox{Arg} \min_{\x \in \T } \Upsilon (\x; \bsig, x_0 )  = \{\x_{\bsig, x_0}\}.
$$
Further   the hypothesis of the Maximum theorem  are satisfied
for the above parametrized optimization problem because of the following steps:
\begin{itemize}
    \item using similar arguments as before (see \eqref{Eqn_integral_ctns}), Dominated convergence theorem twice and the uniform upper bounds of \eqref{Eqn_upperbounds}, one can  prove the joint sequential continuity\footnote{As $\| \x_n -\x \|_\infty \to 0, \bsig_n \rwc \bsig$ and $ x_{0n} \to x_0$, we have  
    $\Upsilon( \x_n; \bsig_n, x_{0n}) \to \Upsilon( \x; \bsig, x_{0})$. } of $\Upsilon$ on $\T \times \Sscr \times \I$;
    \item the domain of optimization  is the same  for any $(\bsig, x_0) \in \Sscr \times \I$ and equals $\T$---the  class $\T$ is proved to be compact under uniform topology in part (a)---thus we have a constant and hence continuous compact correspondence, $(\bsig, x_0) \mapsto \T$. 

    \item further by uniqueness,  the minimizer correspondence $a_\Upsilon^*$ has unique element $\x_{\bsig, x_0}$  for every $(\bsig, x_0) \in \Sscr \times \I $---thus one can view  $a_\Upsilon^*$ as a  single-valued  function (and not correspondence);
\end{itemize}
Therefore by the Maximum theorem, and its corollaries (see \cite{berge1877topological}), we have continuity of the minimizer function $a_\Upsilon^*$ wrt $(\bsig, x_0)$ and the minimizers are exactly the relaxed trajectories. In all,  we have  the continuity of the relaxed trajectories  in the  uniform topology  and so  \eqref{Eqn_thm1_partb} follows.  
\eop


\subsection*{Proof of Theorem \ref{Thm_existence_relx_cont}, Part (a)}
\label{App_thm3}Define $K:= \max \{K_f, K_L \}$ (see \ref{assum_a1}-\ref{assum_a2} for $K_f, K_L$). 
Using exactly the similar arguments as in proof of  \eqref{Eqn_integral_ctns}, we have, for  each  $[0, t] \subset T $
\begin{eqnarray}
\label{Eqn_Lr_ctns}
\int_0^t L_{r}(s,x_{\bsig_n, x_{0n}}(s),\sigma_n(s))\,ds
\to
\int_0^t L_r(s,x_{\bsig, x_{0}}(s), \sigma(s))\,ds, \quad  \mbox{ for all } t \in T, 
\end{eqnarray}
this time 
using the  continuity   of $L_r$ given by \ref{assum_a2} and the upper  bound $\bar z$ of \eqref{Eqn_upperbounds}, which in turn is derived using \ref{assum_a1}---observe  $L_r$ can be   bounded as below, further by   \ref{assum_a0}, 
$$
|L_r(s,x_{\bsig_n, x_{0n}} (s),\sigma_n(s))| \le \max_{t \in T, \  |x| \le \bar z,  \  u \in U }  | L_r(t, x, u) | < \infty,   \  \mbox{ for any }
n, s. $$ 
Let $\x_n :=\x_{\bsig_n, x_{0n}}$ and $\x := \x_{\bsig, x_0}$;
similarly  let $\y_n$ and $\y$ represent the  corresponding max-trajectories   $\y_{\bsig_n,x_{0n}}$ and $ \y_{\bsig,x_{0}}  $ defined in  \eqref{Eqn_y_defn}.
By  Theorem~\ref{thm:relaxed_controls_refined}.(b),  for every $\epsilon>0$, there exists an  $N_\epsilon >0$ such that,
$|| \x_n - \x||_{\infty}   < \nicefrac{\epsilon}{K}$  for all $n \ge  N_\epsilon$. 



Now, consider any $ t \in  T$.
By compactness of $[0, t]$ and continuity of $L_{mx}$ using \ref{assum_a2},  there exists $s^*_n \in [0,t]$ such that
$
y_n(t)= \sup_{s \in [0,t] }L_{mx}(s, x_n (s)) = L_{mx}(s^*_n, x_n(s_n^*)).
 $
Then using \ref{assum_a2},
\begin{eqnarray*}
y_n(t) - y(t)  &=&   L_{mx}(s^*_n, x_n(s_n^*)) - y(t)  \le   L_{mx}(s^*_n, x_n(s_n^*)) - L_{mx}(s^*_n, x(s^*_n))  \\
     &\le& K  | x_n(s^*_n) - x(s^*_n) | \ 
    \le \  K      \|   \x_n -\x \|_\infty < \epsilon,  \mbox{ for all } n > N_\epsilon. 
\end{eqnarray*}
Since $t \in T$ is arbitrary, we have
$\| \y_n - \y\|_\infty <  \epsilon,  \mbox{ for all } n > N_\epsilon.$
Again,  as $\epsilon > 0$ is arbitrary, this completes the proof of part (a)---also see  \eqref{Eqn_Lr_ctns}. 


{\bf Part (b):}
By part (a),  the objective function in \eqref{Eqn_combined_problem_relaxed} is  continuous  wrt  $(\x, \bsig, x_0) \in \A$  and then   part (b) follows by  the compactness of $\A$ from Theorem \ref{thm:relaxed_controls_refined}.(a) and the Weierstrass theorem.  \eop



\subsection*{Proof of Lemma \ref{Lem_exist_optimal_control}}
\label{app_lemma_exitence}
\textbf{Part (i):} We show that the RHS of the  $\y_\bsig^\delta$-ODE in \eqref{Eqn_final_problem_compact_relaxed}  satisfies the Lipschitz continuity and uniform boundedness conditions of \ref{assum_a1}.
 
 {\bf Lipschitz continuity:}
Let the RHS of the $\y_\bsig^\delta$-ODE in \eqref{Eqn_final_problem_compact_relaxed} be represented compactly by, 
$
F(s,x,y,u) := \big ( \Delta_{mx} (s, x, u)  \big )^+ \psi_\delta(L_{mx} (s,x)-y).
$
Further,
we have already shown in Appendix \ref{App_relaxed_trajectories}, while proving Theorem \ref{thm:relaxed_controls_refined},   that $|x(t)| \le \bar z$  of \eqref{Eqn_upperbounds}, under \ref{assum_a1} for all $\bsig \in \Sscr$, $t \in T$ and $x_0 \in \I$. Also observe $\x_\bsig$ ODE is decoupled, while only $\y_\bsig^\delta$ solution is coupled to that of $\x_\bsig$. 
\textit{Thus,  
one can replace 
$F(s, x, y, u) = F(s, x_z, y, u)$ without  altering the problem, where the $i$-th component of $x_z$  is given by,
$$(x_z)_i := \max \{ -\bar{z}, \   \min \{ \bar z, x_i\} \}; \mbox{ also note here, } |x_z| \le \bar z \mbox{ and }  |x_z-x_z'| \le |x-x'|.
$$}
Further  by definition, 
$|\psi_\delta(d) - \psi_\delta(d')| \le  \delta^{-1} |d-d'|$ and $\psi_\delta(d) \in [0,1]$, for all $d$. 
Now consider any  $x,x' \in \mathbb{R}^n$ and $ y,y' \in \mathbb{R}$. Then, using $\bar{z}$   of   \eqref{Eqn_upperbounds}  and assumptions \ref{assum_a1}-\ref{assum_a3},  $F$ is Lipschitz jointly continuous in $(x,y)$, because: 
\begin{eqnarray*}
  && \hspace{-2mm}   |F(s,x_z,y, u) - F(s, x'_z,y', u)| \\
&& \le \Big| \left(\Delta_{mx}(s,x_z, u)\right)^+   - \left(\Delta_{mx}(s,x'_z,u ) \right)^+ \Big| \psi_\delta\big (L_{mx}(s,x_z)-y \big ) \\
&& \quad + \Big| \psi_\delta(L_{mx}(s,x_z)-y)  - \psi_\delta(L_{mx}(s,x_z')-y') \Big|  \left(\Delta_{mx}(s,x'_z,u)\right)^+ \\
&& \le \Big| \Delta_{mx}(s,x_z,u)   - \Delta_{mx}(s,x_z',u)  \Big| \psi_\delta(L_{mx}(s,x_z)-y)    \qquad  (\mbox{as } |a^+ - b^+| \le |a-b|) \\
&& \quad + \left (\Big|  L_{mx}(s,x_z)   -  L_{mx}(s,x'_z) \Big| + \Big|y - y'\Big| \right ) \delta^{-1}K_\Delta(1 + \bar{z}) \\
&& \le K_\Delta |x_z-x'_z| +  \left( K_L|x_z-x'_z| + |y-y'|  \right) \delta^{-1} K_\Delta(1 + \bar{z}) \quad\le \quad K_F \max \{ |x -x'|,  |y-y'| \}, 
\end{eqnarray*}
where $K_F:= K_\Delta \max\{  1 +  K_L\delta^{-1}(1 +\bar{z}) , \delta^{-1} (1 + \bar{z})\}$ is the Lipschitz constant, and we used the  max-norm  for the ordered pair $(x,y)$.


\textbf{Uniform boundedness:}  
Since 
  $\psi_\delta \le 1$, we have, 
$|F(s,x_z,y, u)| \le |\Delta_{mx}(s,x_z, u)|.$
Again using $\bar{z}$  of \eqref{Eqn_upperbounds}   and \ref{assum_a3}, we have 
$|\Delta_{mx}(s,x_z, u)| \le K_\Delta (1 +\bar{z})$. Therefore, $|F(s,x_z,y)| \le K_\Delta (1 +\bar{z})$.

Thus, the joint trajectories of ODEs 
$(\x_\bsig, \y_\bsig^\delta)$ satisfy both Lipschitz continuity and linear growth conditions of \ref{assum_a1}, after replacing $x$ with $(x, y)$ and  $f$ with $(f, F)$. Hence the result follows by  Theorem \ref{thm:relaxed_controls_refined}.(b). 

\textbf{Part (ii):} Using the    results of \cite{roxin1962existence},  we  first prove the existence of solution for, 
%
\begin{eqnarray}
    \label{Eqn_smooth_pure}
\sup_{\u \in \U} W(\x_\u,  \y_\u^\delta; \u)\quad \text{subject to }  \eqref{Eqn_relaxed_dynamics_refined} \mbox{ and } \eqref{eq:ydelta}, \mbox{ with } y_\bsig^\delta(0) = x_\bsig(0)=x_0, \end{eqnarray}
 obtained  by 
 replacing the domain $\Sscr$ with smaller  $\U$
 in \eqref{Eqn_final_problem_compact_relaxed}. Towards this, we first convert the above  into a Mayer-type problem (with only terminal cost)---applying  a standard technique, we augment the state with a new component  
$z_{\u}(t) := \int_0^{t}  L_r(s, x_{\u}(s), u(s)) ds,$  for all  $t \in [0, t_1]$
and equivalently solve $ \sup_{\u \in  \U} \left(z_{\u}(t_1) -   y^\delta_\u(t_1)  - \Psi(x(t_1))\right)$. All the  assumptions from \cite[Assumptions (i)-(vii)]{roxin1962existence} are satisfied in our setup as  below:
\\
$\bullet$ Assumption (i) follows from \ref{assum_a0} and (v), (vi) are satisfied  by definition of $\U$ in \eqref{Eqn_Controls_space}. 
%, with finite horizon $[0,t_1]$.
\\
$\bullet$
     Assumption (ii) is satisfied because, over a finite horizon, and under assumptions \ref{assum_a1}-\ref{assum_a2},  functions $f$ and $L_r$ are continuous and hence integrable in $t$ for all $(x, u) \in \mathbb{R}^n \times U$. From assumption \ref{assum_a3}, the right-hand side of equation \eqref{eq:ydelta} is well-defined and RHS of ODE \eqref{eq:ydelta} also satisfy assumption (ii) of \cite{roxin1962existence}.\\
$\bullet$ 
      The remaining assumptions (iii), (iv) and (vii) are directly satisfied by assumptions \ref{assum_a1} and \ref{assum_a3}-\ref{assum_a5}. 

Thus by \cite{roxin1962existence}, there  exists a  $\u^*_\delta \in \U$  that is optimal for \eqref{Eqn_smooth_pure}. The denseness of Lemma~\ref{lemma_space_compact} and the  continuity of $\bsig \mapsto W(\x_\bsig, \y_\bsig^\delta; \bsig)$,  provided by  Theorem \ref{Thm_existence_relx_cont} and part (i),  implies the following:    for every $\epsilon > 0$, there exists a   $\u_\epsilon \in \U$ such that,
$ W(\x_{\u_\epsilon}, \y_{\u_\epsilon}^\delta;\u_\epsilon) \leq \vr^{\delta} + \epsilon$, for  $\vr^\delta$ of \eqref{Eqn_final_problem_compact_relaxed}.
Further since $\U \subset \Sscr$, we have: 
$$
\vr^{\delta}  \geq W(\x_{\u^*_\delta}, \y_{\u^*_\delta}^\delta;\u^*_\delta) 
\geq W(\x_{\u_\epsilon}, \y_{\u_\epsilon}^\delta;\u_\epsilon)
\geq \vr^{\delta} - \epsilon. 
$$
By letting  $\epsilon \to 0$, we have   $W(\x_{\u^*_\delta}, \y_{\u^*_\delta}^\delta;\u^*_\delta) = \vr^{\delta}$, and so, $\u^*_\delta$ is also optimal for~\eqref{Eqn_final_problem_compact_relaxed}.
\eop

\subsection*{Proof of Theorem \ref{Thm_ydel_convg}}
\label{app_thm_y_ctny}


 \textbf{Part (ii):} The result is derived using
 mathematical induction on $i$: with  $\II_\ell := (\Up_\ell, \Dw_\ell) \cup [\Dw_\ell, \Up_{\ell+1}]$ for each $\ell$,  we prove \eqref{Eqn_Sw}     for all $t \in   \II_i$,  assuming the  same for  all previous intervals, i.e., for all $t \in \cup_{\ell < i} \II_\ell$. 
 
%  The proof in each induction step  is derived using the following  two major parts:
% \begin{enumerate}
%     \item [1.]   We  will show that $L_{mx}(t) \in [y^\delta(t) - \delta, y^\delta(t)]$ and   $y^0(t) \in [L_{mx}(t), y^\delta(t)]$, for all $t \in \cup_i(\Up_i, \Dw_i)$. 
% \item [2.] Second step is to show that   
% $y^\delta(t) = y^\delta (\Dw_i)$ and $y^0(t) = y^0 (\Dw_i)$ for  $t \in [\Dw_i, \Up_{i+1}]$ for any $i$ (both the trajectories remain constant in these intervals). 
% $y^\delta(t) - \delta(t) > x $ and $y^\delta \in [y, y + \delta]$, for all $t \in (\Dw_i, \Up_{i+1})$,. Thus, $y $ and $y^\delta$ trajectories  remain constant within this interval.
%\end{enumerate}
Further we will see that the initial step (or the base case) of the induction proof follows exactly as any  other inductive step;
%---if  $\Up_1 = 0$,  the initial step  is merged with  part (a), otherwise with part (b); 
these details are evident in the proof given below. 
 
{\bf Step 1:} Consider   $(\Up_i, \Dw_i)$  for some  $i$ and assume  \eqref{Eqn_Sw} is satisfied for all $t \le \Up_i$, which implies the following at $t = \Up_i$:
\begin{equation}
y^0(\Up_i) \in [y^\delta(\Up_i) - \delta, y^\delta(\Up_i)] \mbox{ and  further by definition of $\Up_i$, } L_{mx}(\Up_i)  \ge y^\delta(\Up_i) - \delta.
\label{Eqn_y0_at_ui}
\end{equation}
Observe the above conditions are satisfied even for the first interval,   when $\Up_1 = 0$, as the initial conditions  are  $y^0(0) = y^\delta(0) = L_{mx}(0)$ and the proof of the induction step remains the same even for such  an initial step. Hence we provide one proof as below. 


To begin with, from \eqref{Eqn_definition_ui_di}, for all $ t \in (\Up_i, \Dw_i)$, we have 
  $ L_{mx}(t) >  y^\delta (t) - \delta$ and  $\bdot{L}_{mx}(t) >0$. Thus by definition of $y^0(t)$ in \eqref{Eqn_y_defn},
  \begin{eqnarray}
  \label{Eqn_one_dir}
      y^0(t) \ge L_{mx}(t) >  y^\delta (t) - \delta \mbox{ for all } t \in (\Up_i, \Dw_i). 
  \end{eqnarray}
Firstly, say  $y^0$ remains constant:    $y^0(t) = y^0 (\Up_i)$,   for all  $ t \in (\Up_i, \Dw_i)$.
Then  by non-decreasing nature of $y^\delta$ and \eqref{Eqn_y0_at_ui}, we have $y^\delta (t) \ge y^\delta (\Up_i) \ge y^0(\Up_i) = y^0(t)$, for all $t \in (\Up_i, \Dw_i)$.  Hence \eqref{Eqn_Sw} is satisfied  for all $t <  \Dw_i$, proving the inductive step for this sub-case, see also \eqref{Eqn_one_dir}. 
  
Now  consider the next sub case when $y^0 (\tau) > y^0(\Up_i)$ for some $\tau  \in  (\Up_i, \Dw_i)$.
As  $\bdot{L}_{mx}(t) >0$  in $(\Up_i, \Dw_i)$ interval,    $L_{mx} (t)$ is strictly increasing and thus by definition of $y^0(t)$ in \eqref{Eqn_y_defn}, 
  there exists an  $ s \in  [\Up_i, \Dw_i)$ such that (one can have $(\Up_i, s)$ empty if $s=\Up_i$),
\begin{eqnarray}
\label{Eqn_y0_in_ui_to_di}
 \hspace{10mm}   y^0(\Up_i) =  y^0(t) > L_{mx}(t) \mbox{ for  } t \in (\Up_i, s) \mbox{ and } \ 
    y^0(t) =  L_{mx}(t),  \mbox{ for all } t \in  [s, \Dw_i).
\end{eqnarray}
 
   

From the definitions in \eqref{Eqn_definition_ui_di},
   the derivative  $\bdot{y}^\delta (t) > 0$,  for all $t \in (\Up_i, \Dw_i)$; further by \eqref{eq:ydelta}, we have  $0< \bdot{y}^\delta (t) \le \bdot{L}_{mx}(t)$. By virtue of the smaller derivative for~$y^\delta$, we only have  the following two possibilities in this interval and the sub-case of \eqref{Eqn_y0_in_ui_to_di}. 

\begin{enumerate}[(a)]
    \item  The trajectory $y^\delta$ remain bigger, i.e.,  $y^\delta(t) > L_{mx}(t)$ for all $t \in (\Up_i, \Dw_i)$.   
    Since $y^\delta$ is non-decreasing,   we have 
    $$y^0(t) = y^0(\Up_i) \le y^\delta (\Up_i) \le y^\delta (t) \mbox{ for all }t \in (\Up_i, s),  \mbox{ for } s   \mbox{ of }\eqref{Eqn_y0_in_ui_to_di}, $$  and for  $t \in [s, \Dw_i)$, we again have 
    $y^\delta (t) > L_{mx}(t) = y^0(t)$. In all, \eqref{Eqn_Sw} is again satisfied in  $(\Up_i, \Dw_i)$ for this condition also, see \eqref{Eqn_one_dir}. 
\item  There exists an $s' \in (\Up_i, \Dw_{i})$ such that   $y^\delta(t) > L_{mx}(t)$ for $t \in (\Up_i, s')$ and $y^\delta(t) = L_{mx}(t)$  for $t\in [s', \Dw_i)$. 

Now for $t < s'$, \eqref{Eqn_Sw}  is satisfied as in previous $(a)$ case; 
by continuity $y^\delta(s') \ge y^0(s')$,  and at $s'$,  we have 
$L_{mx}(s') \le y^0(s') \le y^\delta(s') = L_{mx}(s')$, implying $L_{mx}(s') = y^\delta(s') = y^0(s')$;  finally for $t \in  (s' , \Dw_i)$,  \eqref{Eqn_Sw} is satisfied with
$y^\delta (t) = L_{mx}(t) = y^0(t)$  (again using \eqref{Eqn_one_dir} and note here that, we will have  $s \le s'$). 
 

 
\end{enumerate}
In summary,  \eqref{Eqn_Sw} is satisfied for all $t \le \Dw_i$,  by continuity and further using the induction assumption.


{\bf {Step 2:}} Now consider  $(\Dw_i, \Up_{i+1})$  for some  $i$ and assume  \eqref{Eqn_Sw} is satisfied for all $t \le \Dw_i$, which implies: 
$$
y^\delta (\Dw_i)  \in  [y^0(\Dw_i),  \  y^0(\Dw_i) +\delta] \mbox{ and by definition \eqref{Eqn_definition_ui_di}, } y^\delta (\Dw_i) -\delta \le  L_{mx}(\Dw_i).
$$
Again the initial step also satisfies the above because of the  initial conditions $y^0(0) = y^\delta(0) = L_{mx}(0)$, even when  $\Up_1 > 0 = \Dw_0$. 

For any $t \in [\Dw_{i}, \Up_{i+1}]$, by definition $\bdot{y}^\delta = 0$ and 
\textit{thus $y^\delta (t) = y^\delta (\Dw_{i}^\delta)$, for all such $t$.}  
%

 We further claim  $L_{mx} (t) \le  y^\delta (t) - \delta$ for  $t \in (\Dw_{i}, \Up_{i+1})$. For the purpose of contradiction, assume at some $\tau \in ( \Dw_i, \Up_{i+1})$, we have $L_{mx} (t) >  y^\delta (t) - \delta$. Now define $s := \sup \{ t < \tau:  L_{mx} (t) = y^\delta (t) - \delta\}$. Clearly by continuity $s < \tau$ and   $ L_{mx} (t) >  y^\delta (t) - \delta$  for all $t \in (s, \tau]$. But  by mean value theorem implies the existence of a $s' \in (s, \tau)$   where $\bdot{L}_{mx} (s') > 0$ (as $y^\delta $ is constant here), which contracts the definition of $\Up_{i+1}$, as $s' <\tau < \Up_{i+1}$. 
%This implies by definition of $\Up_{i+1}$ in \eqref{Eqn_definition_ui_di} and continuity that  $L_{mx} (\Up_{i+1}) =  y^\delta (\Up_{i+1}) - \delta$. 
 And hence       $L_{mx} (t) \le  y^\delta (t) - \delta$  and  $y^\delta (t) = y^\delta (\Dw_i)$ for all $t \in [\Dw_{i}, \Up_{i+1}]$, implying
\begin{eqnarray*}
y^\delta (t ) - \delta =  y^\delta (\Dw_i ) - \delta \le  y^0 (\Dw_{i})  \le    y^0(t)  &= & \max \left  \{ y^0 (\Dw_i), \max_{s \in [\Dw_i, t]} L_{mx} (s) \right  \}  \\
 &\le& \max \left  \{ y^\delta (\Dw_i), \max_{s \in [\Dw_i, t]} y^\delta  (s) -\delta \right  \} =  y^\delta (\Dw_i)  =  y^\delta (t).
\end{eqnarray*}
%implying $y^0 (t) \in [y^\delta (t)-\delta, y^\delta ]$. 
%
\ignore {
this inequality is strictly negated, this means 


Further, $L_{mx} (t) < y^\delta (t) - \delta$ for $t \in (\Dw_{i}, \Up_{i+1})$, by definition of $\Up_i$ in \eqref{Eqn_definition_ui_di}. Therefore,  
 \begin{eqnarray*}
     y^0(t) \ge y^0 (\Dw_i) \ge y^\delta (\Dw_i ) - \delta = y^\delta (t)-\delta  > L_{mx}(t), \mbox{ for all such } t   
 \end{eqnarray*}
 implying $\y^0$ trajectory never meets $\x$ trajectory or that $y^0(t) = y^0 (\Dw_i)$ for $t \in (\Dw_{i}, \Up_{i+1})$.



  


 {\color{red} We have $y^\delta (\Dw_i) -\delta \le  L_{mx}(\Dw_i)$. For any $t \in [\Dw_{i}, \Up_{i+1}]$, by definition $\bdot{y}^\delta = 0$ and 
thus $y^\delta (t) = y^\delta (\Dw_{i}^\delta)$, for all  $t$.  Thus, for all $t \in [\Dw_{i}, \Up_{i+1}]$
\begin{eqnarray*}
     y^0(t) \ge y^0 (\Dw_i) \ge  L_{mx}(\Dw_i)\ge y^\delta (\Dw_i ) - \delta  = y^\delta (t ) - \delta. 
 \end{eqnarray*}
This implies that $ y^0(t) \ge y^\delta (t ) - \delta$, for all $t \in [\Dw_{i}, \Up_{i+1}]$. 

Now, also observe that $y^\delta$ is constant and $y^\delta (\Dw_{i}^\delta) \ge  y^0(\Dw_{i}^\delta)$ with $y^0$ is non-decreasing function. Also, 
for all $t \in [\Dw_{i}, \Up_{i+1}]$,  we have $x(t) < y^0(t)$. This implies $y^0(t) \le y^\delta(t)$. }


}%
 %
 Hence $y^0 (t) \in [y^\delta (t)-\delta, y^\delta ]$ and   the comparison status at $\Dw_i$ continues for all $t \in [\Dw_i, \Up_{i+1}]$,   and so \eqref{Eqn_Sw} is satisfied for all $t \le \Up_{i+1}$, after using the induction assumption. 
\eop

\Remove{
\section*{Proof of Lemma \ref{Lem_value_fun_ineq}}
\label{App_lem_dp}
From \eqref{Eqn_value_fun}, for any given $\delta>0$, it is possible to   choose a control $\u^1 \in \mathcal{U}([r, t_1])$ such that
\begin{equation}
    \int_r^{t_1} L\left(s, x^1(s), u^1(s)\right) d s - \vee_{r, z_\u}^{t_1} (\x^1) +\Psi\left( x^1\left(T\right)\right) \geq v(r, x(r), z_\u)+\delta,
    \label{Eqn_value_supremum_property}
\end{equation}
where  $\x^1$ is the state trajectory for control $\u^1$ and 
$x^1(s)$  is the state  at time $s$ with initial condition ($r, x(r), z_\u$). Such a control $\u^1$ is called $\delta$-optimal for \eqref{Eqn_value_fun}. Define an admissible control $\tilde{\u} \in \mathcal{U}(\tau, t_1)$ by
$\tilde{u}(s) = u(s) \mathds{1}_{\{s \leq r \}} + u^1(s)\mathds{1}_{\{s >r \}},  \mbox{ for all } s \in [\tau, t_1]$. 
%$$
% \tilde{u}(s)=\left\{\begin{array}{l}
% u(s), s \leq r \\
% u^1(s), s>r, 
% \end{array}\right. \mbox{ for all } s \in [\tau, t_1]. 
% $$
Let $\tilde{\x}$  be the state trajectory corresponding to $\tilde{\u}$ with initial condition $(\tau, x)$. We have
$$
\begin{aligned}
v(\tau, x,y) & \geq J(\tau, x,y ; \tilde{\u})  =\int_\tau^{t_1} L_r(s, \tilde{x}(s), \tilde{u}(s)) d s - \vee_{\tau, y}^{t_1} (\tilde{\x})
+\Psi( \tilde{x}(t_1)) \\
 & =\int_\tau^r L_r(s, x(s), u(s)) d s+\int_r^{t_1} L\left(s, x^1(s), u^1(s)\right) d s  +\Psi\left( x^1\left(t_1\right)\right) \\
 & \hspace{10mm}-   \max \left\{ y, \sup_{t \in [\tau, r]} L_{mx}(t, x(t)), \sup_{t \in [r, t_1]} L_{mx}(t, x^1(t)) \right\} \\
 & {=}\int_\tau^r L_r(s, x(s), u(s)) d s+\int_r^{t_1} L\left(s, x^1(s), u^1(s)\right) d s +\Psi\left( x^1\left(t_1\right)\right) \\
 & \hspace{10mm} - \max \left\{ z_\u, \sup_{t \in [r, t_1]} L_{mx}(t, x^1(t)) \right\} \quad \left(\because \max \{ y, \sup_{t \in [\tau, r]} L_{mx}(t, x(t))\} = z_\u\right)\\ 
 & {=}\int_\tau^r L_r(s, x(s), u(s)) d s+\int_r^{t_1} L\left(s, x^1(s), u^1(s)\right) d s - \vee_{r, z_\u}^{t_1} (\x^1) +\Psi\left( x^1\left(t_1\right)\right) \\
& {\geq} \int_\tau^r L_r(s, x(s), u(s)) d s+ v(r, x(r), z_\u)+\delta   \qquad \ (\mbox{using \eqref{Eqn_value_supremum_property}}).
\end{aligned}
$$
% Observe that $\Gamma_r({x})(r)= \Gamma_r({x}^1)(r)$ and thus equality $`a'$ is true. 
As $\delta>0$ is arbitrary,  the  inequality \eqref{Eqn_value_ineq1} is satisfied. 
\eop}



% {\color{blue} 
% {\bf Step 2:} Now consider  $(\Dw_i, \Up_{i+1})$  for some  $i$ and assume  \eqref{Eqn_Sw} is satisfied for all $t \le \Dw_i$, which implies: 
% $$
% y^0(\Dw_i)  = [y^\delta(\Dw_i),  y^\delta(\Dw_i) +\delta] \mbox{ and } y^\delta (\Dw_i) -\delta < x(\Dw_i).
% $$
% Again the initial step also satisfies the above because of the given initial conditions, when  $\Up_1 > 0 = \Dw_0$

% $\mbox{For any } t \in [\Dw_{i}, \Up_{i+1}], \ \dot{y}^\delta (t) = 0, \mbox{ as  } \dot{x}(t) \le  0 \mbox{ or } x(t) \le  y^\delta (t) - \delta.$ 
%  Thus, $y^\delta (t) = y^\delta (\Dw_{i}^\delta)$, for all such $t$. Also, observe a) $y^\delta (\Dw_{i}^\delta) - y^0(\Dw_{i}^\delta) \le \delta$, b) $y^\delta (\Up_{i+1}^\delta)-\delta = x(\Up_{i+1}^\delta) $ and, c) $y^0$ is non decreasing function. 

% Thus, 
% \begin{eqnarray*}
%     y^\delta(t) &=& y^\delta (\Dw_{i}^\delta), \mbox{ for all } t \in [ \Dw_{i}^\delta, \Up_{i+1}^\delta], \mbox{ and } \\
%     y^0(t) &=& y^0 (\Dw_{i}^\delta), \mbox{ for all } t \in [ \Dw_{i}^\delta, \Up_{i+1}^\delta]. 
% \end{eqnarray*}
% In summary, $y^\delta(t) \in [y^0(t), y^0(t) + \delta]$  for $t \in [\Dw_i, \Up_{i+1}]$,     and hence \eqref{Eqn_Sw} is satisfied for all $t \le \Up_{i+1}$, after using the induction assumption.





% %When  $\Up_{i+1} > 0$, the initial step will be $( \Dw_i, \Up_{i+1})$, and the  corresponding initial conditions  satisfied again and the proof is exactly same as for any other $i$.



% {\bf Step 2:} Now consider  $(\Dw_i, \Up_{i+1})$  for some  $i$ and assume  \eqref{Eqn_Sw} is satisfied for all $t \le \Dw_i$, which implies: 
% $$
% y^0(\Dw_i)  = [y^\delta(\Dw_i),  y^\delta(\Dw_i) +\delta] \mbox{ and } y^\delta (\Dw_i) -\delta < x(\Dw_i).
% $$
% Again the initial step also satisfies the above because of the given initial conditions, when  $\Up_1 > 0 = \Dw_0$

% For any $t \in [\Dw_{i}, \Up_{i+1}]$, by definition $\bdot{y}^\delta = 0$ and 
% thus $y^\delta (t) = y^\delta (\Dw_{i}^\delta)$, for all such $t$.  Further, $x (t) < y^\delta (t) - \delta$ for $t \in (\Dw_{i}, \Up_{i+1})$, by definition of $\Up_i$ in \eqref{Eqn_definition_ui_di}. Therefore,  
%  \begin{eqnarray*}
%      y^0(t) \ge y^0 (\Dw_i) \ge y^\delta (\Dw_i ) - \delta = y^\delta (t)-\delta  > x(t), \mbox{ for all such } t   
%  \end{eqnarray*}
%  implying $y^0$ trajectory never meets $x$ trajectory or that $y^0(t) = y^0 (\Dw_i)$ for $t \in (\Dw_{i}, \Up_{i+1})$.
 
% %  Also, observe: a) $y^\delta (\Dw_{i}^\delta) - y^0(\Dw_{i}^\delta) \le \delta$,  b) $y^\delta (\Up_{i+1})-\delta = x(\Up_{i+1}) $, and c) $y^0$ is a  non decreasing function. 

% % Thus, 
% % \begin{eqnarray*}
% %     y^\delta(t) &=& y^\delta (\Dw_{i}^\delta), \mbox{ for all } t \in [ \Dw_{i}^\delta, \Up_{i+1}], \mbox{ and } \\
% %     y^0(t) &=& y^0 (\Dw_{i}^\delta), \mbox{ for all } t \in [ \Dw_{i}^\delta, \Up_{i+1}]. 
% % \end{eqnarray*}
% In summary the comparison status at $\Dw_i$ continues for all $t \in [\Dw_i, \Up_{i+1}]$, hence $y^\delta(t) \in [y^0(t), y^0(t) + \delta]$  for such $t$,  and so \eqref{Eqn_Sw} is satisfied for all $t \le \Up_{i+1}$, after using the induction assumption. \eop
% %When  $\Up_{i+1} > 0$, the initial step will be $( \Dw_i, \Up_{i+1})$, and the  corresponding initial conditions  satisfied again and the proof is exactly same as for any other $i$. 


% }
  
% \sout{Let $\mathscr{P} (\X) :=  \{ A \subset \X : A \ne \emptyset \}$, represent the class of non-empty subsets of $\X$ and let $\I$ represent a non-empty compact subset of  $\mathbb R$ that represents the set of initial conditions.  } Let $C(T)$ be the space of continuous real-valued functions on $T$ and consider the following class of  relaxed  trajectories controls and initial conditions:
% \begin{equation}
%    \A :=\bigg  \{ (\x,   \sigma , x_0 )  \in  C(T)  \times \Sscr  \times \I: \x \mbox{ is solution of \eqref{Eqn_relaxed_dynamics_refined}  under   } \sigma \mbox{ with }x(0) = x_0   \bigg \},  
% \end{equation}
% where $\I$ is compact subset of $\mathbb{R}^n$. When there is a requirement, we represent the relaxed trajectory $\x$ with $\x_\bsig$ to explicitly indicate the dependence on $\sigma$. 
\ignore{
Part (c) is established using  Weierstrass theorem, however 
one requires more arguments  for the non-standard problem in \eqref{Eqn_combined_problem_relaxed}---mainly to establish continuity of max-trajectory $\y_\bsig = (y_\bsig (t), t \in T)$,  defined point-wise  as below:
\begin{eqnarray}
    y_\bsig(t) :=  \sup_{s \in [0, t] }  L_{mx} (s, x_\bsig (s) )  , \mbox{ for all } t \in T,\label{Eqn_y_defn}
\end{eqnarray}
with respect to $\sigma$. 
This part of the proof is    also provided  in  Appendix \ref{App_relaxed_trajectories}.

The major steps are:
\begin{itemize}
    \item We will first show the conditions of \cite[Theorem VI.1.1]{warga2014optimal} 
    are applicable to  establish parts (a)-(b). 
    % Then we have the following: 
    %  $\A = \A (\Sscr)$ is sequentially compact   and  the mapping of relaxed trajectory $\sigma \mapsto \x_\bsig $ is sequentially continuous, i.e., in the following manner
    % $$
    % \mbox{ if } \sigma_n \rwc \sigma \mbox{ then }   \sup_{t \in T} |x_{\sigma_n} (t) - x_\bsig (t) | \to 0.
    % $$


    \item We next  show that the max trajectory $\y_\bsig$  of \eqref{Eqn_y_defn}  and hence the objective function in \eqref{Eqn_combined_problem} are continuous wrt  $(\x, \bsig, x_0) \in \A$. Then the proof 
    follows by Weierstrass theorem. 
\end{itemize}

Towards applying \cite[Theorem VI.1.1]{warga2014optimal}, we first show that the  problem in \eqref{Eqn_combined_problem} can be typecast as  the problem formulated as in \cite[Chapter VI.0, pg 347]{warga2014optimal}, with following details:

\begin{itemize}

\item We have no constraints on the relaxed trajectories,  thus we set  $g_2 = h_2 \equiv 0$ and $C_2 = \{ w: w (t) =   \mathbb{R}^n \mbox{ for all } t \in T \}$ in the problem formulation of \cite[Section VI.0]{warga2014optimal}.      
 
 
\item We don't have  control parameters in our setup---observe $f$ in \eqref{Eqn_combined_problem} depends only upon $(t, x, u)$ and  is independent of $b$; also  $g_1$ is meant to impose conditions on terminal time $t_1$, we hence   set $h_1 \equiv 0$ and $B_1 = {\mathbb R}$, see also \cite[Chapter III, pp 241]{warga2014optimal}. 

\item Further to obtain continuity also  wrt initial condition $x_0$, we  add  $b:=\nicefrac{x_0}{t_1}$ to $f$ in \eqref{Eqn_combined_problem}  to obtain the function $f$  considered in 
 \cite[Theorem VI.1.1]{warga2014optimal}, we also set $v_0 = 0$, $t_0=0$ in the theorem hypothesis. Observe then the solution of integral equation in page 347 of \cite[Section VI.0]{warga2014optimal} equals:
 \begin{eqnarray*}
     y = F(y, \bsig, b) = 0 + \int_0^{t} \left ( f(\tau, y(\tau), \sigma(\tau) ) + b  \right ) d\tau = \frac{x_0}{t_1} t_1 + \int_0^{t_1} \left ( f(\tau, y(\tau), \sigma(\tau) )    \right ) d\tau
 \end{eqnarray*}

\item Consider  the solution of $\bdot{z} = K (1+z)$ for $K$ given in assumptions \ref{assum_a0}-\ref{assum_a1},  which  equals  $z(t; x_0) =(1+x_0)e^{Kt} -1 $,  for any $t \in T$ and define,
$$\psi (t) := \max_{ z \le z(t; x_0), u \in U, x_0 \in \I }  | f(t, z, u) | \mbox{  for each } t \in T.
$$
Now  
 observe, using standard results in ODEs and assumption \ref{assum_a1},  that for any solution $\x_\bsig$ of ODE \eqref{Eqn_relaxed_dynamics_refined} under any relaxed control $\sigma \in \Sscr$ we have $x_\bsig(t) \le z(t)$  and thus  
\begin{eqnarray*}
    | f(t, x_\bsig (t; x_0), u) | \le \psi (t) \mbox{ for all } t \in T \mbox{ and } \\  \sup_{t, \bsig, x_0} |x_\bsig (t; x_0) | \le \bar z := \sup_{t \in T, x_0 \in \I} |z(t; x_0) |. 
\end{eqnarray*}



 
is defined as $f + x_0$
 
Finally  with  $v_0=0,  t_0=0,   R,  \psi $ and $  V_0 $ of 
   \cite[Theorem VI.1.1]{warga2014optimal} are given respectively by   $0$,   $f$ in \eqref{Eqn_relaxed_dynamics_refined}, $U$, $\psi (t) = (1+x_0)e^{Kt} -1$ and  $\{ x \in \mathbb{R}^n : |x| \le \bar z\}$  and satisfy the required hypothesis with $V  = \mathbb{R}^n $, because of the above mentioned steps and assumptions \ref{assum_a0}-\ref{assum_a2}.   
    
 
\end{itemize}

}






==> intro.tex <==

\section{Introduction}
\label{sec_intro}
Optimal control theory studies the problem of determining a control policy for a dynamical system so as to optimize a prescribed performance criterion over a given time horizon. Classical formulations of optimal control problems typically involve an objective functional that consists of an integral of a running reward together with a terminal reward (see \cite{ fleming2012deterministic, fleming2006controlled, warga2014optimal}). More precisely, for a system governed by the dynamics $\dot{x}(s) = f(s,x(s),u(s))$,  with initial condition $ x(0)=x_0,$
the objective is usually of the form
$J^r(x_0;u) = \int_0^{t_1} L_r(s,x(s),u(s))\,ds + \Psi(x(t_1))$, where $u(s)$ is the control at time $s$, $\Psi(\cdot)$ represents the terminal  cost (or reward) function and $L_r(\cdot, \cdot, \cdot)$  represents the instantaneous cost (or reward) function. 
Such formulations arise naturally in engineering, economics, operations research, and applied mathematics, where the running reward represents the instantaneous performance of the system and the terminal reward captures the reward  associated with the state at the end of the horizon. 

 
While the classical formulation with integral rewards captures the cumulative   performance of the system, in many practical applications it is equally important to account for extreme or peak behavior over the given time horizon. Such peak performance criteria have also been considered in the literature (see \cite{barron1990pontryagin, barron1999viscosity, barron1989bellman, di1999minimax,fialho1999worst, lygeros2004reachability, serea2002discontinuous, vinter2005minimax})---by minimizing the objective functions of the form $J^\infty( x_0; u) := \sup_{s \in [0, t_1]} L_{mx} (s, x(s))$---where $L_{mx} (s, x(s))$, at any time~$s$,     represents the instantaneous value of a certain quantity whose peak value over the horizon needs to be controlled---and solution $x(\cdot)$ is controlled using $u (\cdot)$  as before.  




    Optimal control problems of both of the above-mentioned types have been extensively studied in the literature
 (see e.g., \cite{barron1989bellman, fleming2012deterministic,fleming2006controlled}). 
The value function of these control problems satisfies a Hamilton--Jacobi--Bellman (HJB) partial differential equation that arises from Bellman's dynamic programming principle. The HJB equation provides necessary and sufficient conditions for optimality and characterizes  the value function of the control problem. Alternatively, Pontryagin's maximum principle  provides necessary optimality conditions through a Hamiltonian associated with HJB equation, involving the state and adjoint variables (see e.g., \cite{barron1990pontryagin, fleming2006controlled}). These two techniques  are used to numerically solve both types of control problems mentioned above: (a) problems with integral (or running) rewards; and  (b) problems with $L^\infty$ rewards. 




In several applications, both aspects, the cumulative running performance and the peak levels, play a crucial role and must be controlled simultaneously.
%
For example, in an inventory control problem, if there is a requirement and flexibility to design the inventory capacity, one needs to optimize a combined objective function formed using typical  holding/shortage running costs as well as the peak inventory levels reached during the planning horizon (e.g., see \cite{dhiman2024optimal}). 
%
%there is an important aspect, which needs attention, the physical capacity of the inventory storage -- once constructed, cannot be altered easily. Such a design  is crucial and  thus, naturally leads to formulations where one seeks to jointly optimize cumulative profit while penalizing the peak inventory levels. 
In queueing systems, in a similar way,  the peak congestion levels reached during the operating period impacts an important design aspect,  the capacity of the waiting room (in fact here the peak levels also represent an important quality of service, important from customer standpoint). The  cumulative occupancy, the  cumulative server capacity utilized, etc., represent the typical running costs (e.g., \cite{bauerle2002optimal, malhotra2009feedback}). Our aim again is to provide solutions to such problems  that cater to both the types of costs. 
Similarly, in epidemic control models, the peak number of infected individuals is often of primary concern, as it reflects the maximum burden on the healthcare systems. Again there is a need to control a combined objective function that includes peak-infection levels  and other running costs, like cumulative vaccination costs (see, e.g., \cite{dhiman2023integrative}). 

Motivated by such applications, in this paper, we study a control problem that maximizes a combined  objective function of  the following  form, 
\begin{eqnarray}
    J( x_0;u) &=&   \int_{0}^{t_1} L_r(s, x(s), u(s))ds  + \Psi(x(t_1)) 
    -  \sup_{s \in [0,t_1]} \{ L_{mx} (s, x (s)) \}.
    \label{eqn_objective}
\end{eqnarray}
The above  formulation  can capture a weighted combination of two or more objective functions,  with one of them being  the peak-level reached by a certain quantity during the operating horizon. 
%
In \cite{barron1999viscosity},  Barron  considered a class of optimal control problems where the objective function combines the two criterion in the following manner:
%involves a supremum over time of a function that combines the running cost and an instantaneous penalty term. A representative formulation considered in their work takes the form
\begin{equation}
\sup_{t\in[0,t_1]}
\left\{
\int_t^{t_1} L_r(s,x(s),u(s))\,ds - L_{mx}(t,x(t))
\right\}
+ \Psi(x(t_1)). 
\label{Eqn_barron_obj_fun}
\end{equation}
Such formulations possess a structure that is particularly amenable to the dynamic programming approach and can be solved and analyzed  using a particular form  of HJB equations.
However, the objective in \eqref{Eqn_barron_obj_fun} differs fundamentally from that in \eqref{eqn_objective}. The former optimizes the running maximum of a quantity that, at each intermediate time~$t$, combines the   instantaneous penalty at~$t$ with the cumulative reward from time~$t$ to the end of the horizon $t_1$. 
In contrast, the objective function in \eqref{eqn_objective} combines the running maximum with accumulated rewards in a manner that naturally accommodates multi-objective optimization problems.
  
  





\ignore{
In contrast, the problem considered in this work involves study a general  control problem that involves a combination of a classical integral cost and an $L^\infty$-type peak cost over the entire time horizon. The objective function is given by
\begin{eqnarray}
    J( x_0;u) &=&   \int_{0}^{t_1} L_r(s, x(s), u(s))ds  + \Psi(x(t_1)) 
    -  \sup_{s \in [0,t_1]} \{ L_{mx} (s, x (s)) \}.
    \label{eqn_objective}
\end{eqnarray}
 This formulation generalizes both the classical optimal control problem with integral cost and the supremum-type formulations studied previously in the literature.

It is important to note that the above problem is different from a standard constrained optimal control problem. In a constrained setting, one typically imposes a condition such as 
$$
\sup_{s \in [0,t_1]} L_{mx}(s,x(s)) \leq \kappa, \mbox{ for some } \kappa< \infty, 
$$
and introduces a Lagrange multiplier term to handle this constraint, thereby converting the problem into an unconstrained one. In that case, the multiplier is chosen (or adjusted) so as to enforce the constraint indirectly.  In contrast, in the present formulation \eqref{eqn_objective} the supremum term appears directly in the objective with a fixed weight, and there is no parameter that can be tuned to recover an equivalent constrained problem. Thus, the problem is not a Lagrangian relaxation of a constraint, but instead reflects a genuine trade-off between cumulative performance and peak values, both of which are optimized simultaneously.}

Our first contribution is to establish the existence of suitable solutions  for problems that optimize \eqref{eqn_objective}. To this end,  we adopt the framework of relaxed controls. By exploiting   the well-known compactness and convexity properties of the relaxed control space, we establish the existence of an optimal relaxed control (see e.g.,~\cite{warga2014optimal}). Then  using the  denseness of pure controls in the relaxed control space (see again~\cite{warga2014optimal}), we prove the existence of  a pure control that is $\epsilon$-optimal for the original problem,   for every $\epsilon > 0$.


While these results guarantee existence, they do not directly lead to a tractable method for computing ($\epsilon$) optimal policies. The presence of the $L^\infty$ term introduces significant analytical challenges: the objective becomes non-smooth %\sout{and depends on the entire trajectory of the state process,} 
and it is not clear whether the classical dynamic programming principle applies to this setting.

To address this difficulty, we adopt an approach based on smooth approximations. We first augment the state by introducing an auxiliary variable, $y(t) := \sup_{s \le t}  L_{mx}(s,x(s)) $, that tracks the running maximum along the trajectory. Although this reformulation captures the path-dependent feature, the resulting problem remains non-smooth. We therefore consider a family of smooth problems that approximate the original formulation, leading to standard optimal control problems for which optimal solutions exist and can be computed numerically.
We then show that, as the smoothing parameter tends to zero, the solutions of the smooth problems converge to those of the original problem. This is established in two main steps: (i) the smooth approximate trajectory  converges to the instantaneous maximum trajectory $y(\cdot)$, and (ii) using the Maximum Theorem, the value functions of the smooth control problems converge to that of the original problem.

%{\color{red}Literature survey}

%To address this difficulty, we adopt an alternative approach based on smooth approximations. As a first step, we augment the state by introducing a maximum trajectory that tracks the running maximum along the path. However, even in this augmented formulation, the objective remains non-smooth. We therefore introduce a family of smooth approximations of the problem, leading to standard optimal control formulations for which optimal solutions exist and can be computed numerically. We further show that, as the smoothing parameter tends to zero, the solutions of the regularized problems converge to those of the original problem.


\ignore{
The presence of the supremum term introduces significant analytical challenges. Unlike classical optimal control problems, the $L^\infty$-term depends on the entire trajectory of the state process, and it is not a priori clear whether the classical dynamic programming framework applies.  Thus, we adopt an alternative approach based on relaxed controls. By using the compactness and convexity properties of the relaxed control space, we establish the existence of optimal relaxed controls. Furthermore, using the well-known denseness of pure controls in the relaxed control space, we show that for every $\epsilon>0$, there exists a classical control that is $\epsilon$-optimal for the relaxed problem.


While these results ensure existence and approximation, the non-smoothness induced by the $L^\infty$-term makes the problem computationally challenging.
To overcome this difficulty, we first introduce a maximum trajectory that tracks the running maximum of the $L^\infty$-term along the trajectory.  However, even in this augmented formulation, the objective remains non-smooth.


For computation tractability, we introduce a family of smooth approximations of the maximum trajectory, parameterized by a regularization parameter. These approximations replace the non-smooth maximum trajectory with a smooth surrogate 
 that enables analytical tractability, 
 %The resulting family of smooth control problems admits better structural properties
 allowing us to employ tools from classical optimal control theory. 
Within this framework, we prove the existence of  optimal control  for the smooth control problems and that the corresponding value functions converge, as the smoothing parameter tends to zero, to the value of the original non-smooth problem. Furthermore, we show that optimal solutions of the approximate problems are $\epsilon$-optimal for the original problem, with approximation guarantees that are uniform in the smoothing parameter.



These results collectively provide a systematic and rigorous approach to analyzing optimal control problems involving a combination of integral and peak cost criteria, and extend the applicability of optimal control theory to settings where both cumulative performance and peak behavior must be simultaneously controlled.}


\subsection*{Connection to hard constraint problem} It is important to note here that the  problem \eqref{eqn_objective} is different from a standard constrained  problem as in \cite{ maurer1977optimal, vinter1998necessary}---where one considers optimizing objective function,  $\int_0^{t_1} L_r(s,x(s),u(s))\,ds + \Psi(x(t_1))$, while   imposing a condition such as 
\begin{eqnarray}
   \label{Eqn_hard_constraint} 
\sup_{s \in [0,t_1]} L_{mx}(s,x(s)) \leq \kappa, \mbox{ for some } \kappa< \infty. 
\end{eqnarray}
Such problems are often addressed by introducing a Lagrange multiplier to incorporate the constraint into the objective, thereby transforming the constrained problem into an unconstrained one resembling \eqref{eqn_objective}. One then seeks an appropriate multiplier that guarantees satisfaction of the original constraint (see \cite{clarke2013functional, gollmann2009optimal, malanowski2004second}). In contrast, our problem is solved for a prescribed multiplier, which directly represents the desired trade-off factor. The two problems also differ fundamentally from the standpoint of applications. A formulation with a hard constraint is appropriate when, for example, a resource is subject to a strict upper bound. In contrast, our formulation is applicable when there is flexibility in determining the optimal level of the resource, with the trade-off governed by the prescribed multiplier.

Another closely related class of problems is that of optimal control with state constraints (see \cite[Section 7]{barron1999viscosity})---these problems can also be seen as problems with hard constraint as in \eqref{Eqn_hard_constraint}. 
Once again, for such problems, an appropriate Lagrange multiplier must be selected, whereas our problem seeks a solution for a given multiplier or trade-off factor.

%\sout{Once again, in the standard Lagrange multiplier framework for such problems, the choice of the multiplier plays a crucial role and is typically not known  apriori, needs to be adjusted. In contrast, for any fixed value of the multiplier, representing the required trade-off factor,  the resulting formulation is  a problem of the type \eqref{eqn_objective} considered in this work.} \sout{In this sense, control problems with state constraints can be viewed as leading naturally to the present framework when one considers fixed multipliers.}

Moreover, for optimal control problems with state constraints, it is well known that establishing a viscosity solution framework is, in general, a challenging and unresolved issue (see \cite[page~7]{barron1999viscosity}). The control formulation involving \eqref{eqn_objective} is of comparable complexity due to the presence of the supremum term. We overcome this difficulty by constructing a family of smooth approximating problems that converge to the original problem as the smoothing parameter tends to zero, thereby deriving the solution to the original problem through a suitable limiting argument.

%In contrast, in the present formulation \eqref{eqn_objective} the supremum term appears directly in the objective with a fixed weight, and there is no parameter that can be tuned to recover an equivalent constrained problem. Thus, the problem is not a Lagrangian relaxation of a constraint, but instead reflects a genuine trade-off between cumulative performance and peak values, both of which are optimized simultaneously.

Finally, the control framework developed in this work can be effectively applied to a broad range of real-world problems, including electricity load balancing, queueing systems, inventory control, epidemic control, etc. In this paper, we also investigate a queueing control problem as an example application of the proposed framework, while another example concerning inventory control is studied in \cite{dhiman2024optimal}. In our earlier short paper \cite{dhiman2024optimal}, we focused only on the smooth-approximation framework (one specific example) and presented inventory control application. In contrast, the present paper focuses on the combined problem \eqref{eqn_objective}, establishing the existence of its $\epsilon$-optimal solutions through solutions of a sequence of smooth approximating problems that can be solved using standard techniques --- using the relaxed control framework and applying the Maximum theorem. 

\subsection*{Queueing $L^\infty$ control}
%\sout{We study an example involving a queuing system.   Our aim in this paper is} 
  The aim here is  to study the contrasts in the  designs that cater to the two congestion costs (peak as well as cumulative) with varying degrees of importance. Using the $L^\infty$ smooth approximate framework  developed in this paper, we obtain the required comparison. We basically study the  two different (and extreme) Pareto frontiers, one that trades-off between the peak-congestion levels and the cumulative server utilization, and the second that trades-off between the cumulative congestion levels and the cumulative server utilization.
 

We observe that there is  a significant   reduction in the peak-congestion levels (even up to $27 \%$) when one  includes the latter cost into the optimization problem; however this \textit{improvement is at the expense of the cumulative congestion cost, which degrades significantly ($20 \%$)}.  
%This is in contrast to the inventory control problem} (negligible degradation was observed in  the cumulative costs even after reducing the peak-inventory levels significantly);
%This difference arises probably because the inventory system penalizes deviation of the inventory level on either side of zero level (holding cost for excess and shortage cost for deficiency), requiring a \textit{balance} near zero; however,  the  queueing system lacks such balancing costs.
%
Thus,  the design for  queuing systems must consider the weight factors for  the three costs judiciously and our proposed framework makes it possible to derive the corresponding optimal policy numerically.  
Interestingly, however, when the cumulative 
server utilization is either too small or is too high, there is negligible difference in the 
performance(s) with and without considering the peak-levels into the design.


 \ignore{ 

%  {\color{red}The first contribution  of this paper  is to devise a technique  to solve   the above non-standard  problem. We introduce an auxiliary state variable,  $y(s) := \sup_{t\le s}  |F_t|$ to capture the instantaneous $L^\infty$ term (e.g., represents the maximum  inventory-level reached,  till time $s$ in  the inventory problem) and convert the $L^\infty$ term to   a terminal cost. This  propels the problem into the standard framework, however   induces a new  technical challenge.  When one designs an ordinary differential equation (ODE) representation for the  new state variable,  the dynamics can only be represented with the help of an indicator function involving the state variables.  Such problems require great technical detail, and could probably be handled  using   Filippov kind of solutions (\cite{filippov2013differential}), which could significantly increase the complexity of the problem.  
% We  instead propose an    appropriate smooth approximation for the converted problem. We show that the value function is the unique viscosity solution of the Hamilton Jacobi Bellman (HJB) partial differential equation (PDE) and establish the existence of the optimal policy for the \textit{$L^\infty$ smooth approximate problem.}   The control framework developed in this work   can be effectively applied to a wide range of real-world problems, like electricity load balancing,  queuing systems, etc.  
% We study the inventory and the queueing control problems mentioned in the beginning using the developed framework.}

The presence of the supremum term introduces significant analytical challenges. Unlike classical optimal control problems, the $L^\infty$ component depends on the entire trajectory of the state process and therefore cannot be directly incorporated into the standard dynamic programming framework. To overcome this difficulty, we introduce a maximum trajectory that tracks the running maximum of the $L^\infty$ cost along the trajectory. This augmented state representation allows the problem to be reformulated as a standard optimal control problem in an extended state space.

The reformulated problem admits a dynamic programming characterization, where the corresponding value function satisfies a Hamilton--Jacobi--Bellman equation on the augmented state space. However, the resulting equation is nonstandard due to the presence of a max-type nonlinearity, which introduces additional analytical complexities. To address these issues, we develop a suitable approximation framework that replaces the supremum term by a smooth approximation, enabling the use of classical analytical techniques.

Under appropriate regularity assumptions on the system dynamics and cost functions, we establish the existence of optimal controls and characterize the value function as the unique viscosity solution of the associated Hamilton--Jacobi--Bellman equation. Furthermore, we show that the solutions of the approximating problems converge to the solution of the original problem, thereby providing a rigorous justification for the approximation scheme.

\medskip

\noindent \textbf{Contributions.} The main contributions of this paper are summarized as follows:
\begin{enumerate}
    \item We formulate a class of optimal control problems involving  combination of integral and $L^\infty$ cost criteria, which extends classical formulations in a nontrivial manner.
    
    \item We introduce an augmented state-space representation that transforms the nonstandard problem into an equivalent control problem amenable to dynamic programming \textcolor{blue}{why dp here?}.
    
    \item We derive the associated Hamilton--Jacobi--Bellman equation and establish a viscosity solution characterization of the value function.
      \textcolor{blue}{do we need to say this? and how?}
    \item We propose a smooth approximation scheme for the $L^\infty$ term and prove convergence of the corresponding value functions to that of the original problem.
    
    \item We establish existence of optimal controls and provide a rigorous analytical framework for control problems involving peak-cost objectives.
\end{enumerate}}

\ignore{
Optimal control theory studies the problem of determining a control policy for a dynamical system so as to optimize a prescribed performance criterion over a given time horizon. Classical formulations of optimal control problems typically involve an objective functional that consists of an integral of a running cost together with a terminal cost. More precisely, for a system governed by the dynamics $\dot{x}(t) = f(t,x(t),u(t)), \quad x(\tau)=x,$
the objective is usually of the form
$J(\tau,x;u) = \int_\tau^{t_1} L(t,x(t),u(t))\,dt + \Psi(x(t_1))$.
Such formulations arise naturally in engineering, economics, operations research, and applied mathematics, where the running cost represents the instantaneous performance of the system and the terminal cost captures the desired final state. Optimal control problems of this type have been extensively studied in the literature; see the classical monographs \cite{fleming2012deterministic,fleming2006controlled}. 
Within this framework, the value function of the control problem satisfies a Hamilton--Jacobi--Bellman (HJB) partial differential equation that arises from Bellman's dynamic programming principle. The HJB equation provides necessary and sufficient conditions for optimality and characterizes the value function of the control problem.

The development of optimal control theory has followed two complementary approaches. The first is the variational approach based on Pontryagin's maximum principle, which provides necessary optimality conditions through a Hamiltonian system involving the state and adjoint variables. The second approach is the dynamic programming framework pioneered by Bellman, where the value function satisfies the Hamilton--Jacobi--Bellman equation and optimal policies can be obtained from the maximization of the Hamiltonian. 
Over the past several decades, a large body of literature has investigated such problems for deterministic and stochastic systems, finite and infinite horizon problems, and various types of running and terminal costs.

While the classical formulation with integral costs captures the cumulative performance of the system, many practical applications require the control of extreme or peak values of certain quantities over the time horizon. In several engineering systems, the worst-case or peak value of a variable can be more critical than its cumulative behavior. For instance, in power systems and communication networks it is important to control peak loads or congestion levels; in inventory and production systems large instantaneous backlogs may be undesirable; and in risk-sensitive decision making one often seeks to limit extreme deviations rather than merely minimizing cumulative costs. Such considerations naturally lead to control formulations involving $L^\infty$-type performance criteria.

Motivated by such applications, several authors have studied optimal control problems involving supremum-type objective functions. In particular, Barron and Ishii \cite{barron1999viscosity} considered a class of optimal control problems where the objective involves a supremum over time of a function that combines the running cost and an instantaneous penalty term. A representative formulation considered in their work takes the form
\begin{equation}
\sup_{t\in[\tau,t_1]}
\left\{
\int_t^{t_1} L_r(s,x(s),u(s))\,ds - L_{mx}(t,x(t),u(t))
\right\}
+ \Psi(x(t_1)).
\end{equation}
Such formulations possess a structure that is particularly amenable to the dynamic programming approach. The associated value function satisfies a Hamilton--Jacobi equation that can be analyzed using the viscosity solution framework, and explicit solution representations can sometimes be obtained through Hopf--Lax type formulas. These works provide a rigorous PDE characterization of optimal control problems involving supremum-type criteria.

Despite these developments, the structure considered in the above formulation is somewhat restrictive from the viewpoint of applications. In many practical systems one simultaneously encounters two types of performance objectives: (i) cumulative performance measured through an integral of running rewards, and (ii) constraints or penalties associated with the peak value of a quantity over the entire time horizon. In such situations the decision maker must balance overall system performance with the need to limit extreme deviations. This naturally leads to optimization problems where both types of costs appear together in the objective function.

In this work we study an optimal control problem that involves a weighted combination of a classical integral cost and an $L^\infty$-type peak cost over the entire time horizon. The objective functional is given by
\begin{eqnarray}
    J(\tau, x;u) &=&   \int_{\tau}^{t_1} L_r(s, x(s), u(s))ds  + \Psi(x(t_1)) 
    - \sup_{s \in [\tau,t_1]} \{ L_{mx} (s, x (s)) \}.
\end{eqnarray}
This formulation generalizes both the classical optimal control problem with integral cost and the supremum-type formulations studied previously in the literature. The parameter $\sigma>0$ represents the relative importance assigned to controlling the peak cost compared with maximizing the accumulated running reward.

The presence of the supremum term introduces significant analytical challenges. Unlike classical optimal control problems, the $L^\infty$ component depends on the entire trajectory of the state process and therefore cannot be directly incorporated into the standard dynamic programming framework. To overcome this difficulty, we introduce an auxiliary state variable that tracks the running maximum of the $L_\infty$ cost along the trajectory. This augmented state representation allows the problem to be reformulated as a standard optimal control problem in an extended state space.

Using this reformulation, we establish the dynamic programming principle for the resulting control problem and characterize the associated value function. In particular, we derive the Hamilton--Jacobi--Bellman equation corresponding to the augmented control problem and show that the value function satisfies this equation in the viscosity sense. Furthermore, we provide a verification theorem that characterizes optimal controls in terms of the solution of the HJB equation.

The main contributions of this work can be summarized as follows. First, we introduce a new class of optimal control problems involving arbitrary weighted combinations of integral costs and supremum-type peak costs over the entire horizon. Second, we develop a dynamic programming framework for this problem by augmenting the state space with a variable that captures the running maximum of the $L^\infty$ term. Third, we derive the associated Hamilton--Jacobi--Bellman equation and establish verification results that characterize optimal controls.

The rest of the paper is organized as follows. In Section~\ref{Aux_state}, we reformulate the original problem by introducing an auxiliary state variable that captures the peak cost term. We then establish the dynamic programming principle for the resulting value function. Subsequently, we derive the Hamilton--Jacobi--Bellman equation associated with the control problem and establish a verification theorem that characterizes optimal controls.}

==> smooth_approx_new.tex <==
\section{Approximation by smooth control problems}   
\label{sec_approximation_by_smooth}
The max-trajectory defined in \eqref{Eqn_y_defn} enables rewriting the $L^\infty$-term  in \eqref{Eqn_combined_problem_relaxed}, $\sup_{s \in T} L_{mx}(s, x_\bsig (s))$,  as a terminal cost, since this term  precisely equals $y_{\bsig}(t_1)$. Let the modified objective function be defined as below:
\begin{eqnarray}
    W(\x_\bsig,  \y_\bsig; \bsig) := \int_{0}^{t_1} L_r(t, x_\bsig(t), \sigma (t))dt  + \Psi(x_\bsig(t_1)) -  y_\bsig(t_1). \label{eqn_obj_fun_with_y}
\end{eqnarray}   
Further after careful examination, one can  describe the  dynamics of this max-trajectory, under any given control $\bsig \in \Sscr$, as below (see also \cite{dhiman2024optimal}):
\begin{eqnarray}
\label{Eqn_y_dynamic_compact}
\bdot{y}_\bsig(s)
&=& \bigg ( \Delta_{mx} (s, x_\bsig (s), \sigma(s) )  \bigg  )^+  \mathds{1}_{\{L_{mx}(s, x_{\bsig}(s)) \ge y_{\bsig}(s)\}}  \mbox{ where }    \\
\hspace{5mm}
\Delta_{mx} (s, x(s), \sigma(s)) 
&:= &
\frac{\partial L_{mx}(s, x(s))}{\partial s}  + \frac{\partial L_{mx}(s, x(s))}{\partial x} f(s, x(s), \sigma(s)), 
\nonumber
\end{eqnarray}
due to the following reasons.  
The above dynamics imply that $\y_\bsig$ is non-decreasing and evolves   for $s \in [s_1, s_2] \subset [0, t_1]$, only  when the trajectory $L_{mx}(s,x_\bsig(s))$ meets the current level $y_\bsig(s)$ with a positive derivative i.e, $\Delta_{mx} (s, x_\bsig(s), \sigma(s)) >0$. In this regime, $y_\bsig(s)$ tracks $L_{mx}(s,x_\bsig(s))$ exactly. If for some time $s$,  $\dt{L}_{mx}(s,x_\bsig(s)) < 0$, then $L_{mx}(s,x_\bsig(s))$ decreases below $y_\bsig(s)$ and $\y_\bsig$ remains constant until $L_{mx}(s,x_\bsig(s))$ increases again and catches up $y_\bsig (s)$. Hence, $\y_\bsig$  the solution of \eqref{Eqn_y_dynamic_compact} (when exists),  effectively captures the running maximum of $L_{mx}(s,x_\bsig (s))$ or the max-trajectory \eqref{Eqn_y_defn}, when further the initial conditions are equal,  $x_\bsig(0) = y_\bsig(0)$ (see Figure \ref{Fig_x_y} also).

Thus, if one assumes \eqref{Eqn_y_dynamic_compact} has `good' solution for all  controls  $\bsig \in \Sscr$, then~\eqref{Eqn_combined_problem_relaxed},   can be rewritten as a  `standard' relaxed-control problem  as below (see \eqref{eqn_obj_fun_with_y}):
\begin{eqnarray}
v_r := \sup_{\bsig \in \Sscr} W (\x_\bsig, \y_\bsig;\bsig) \quad \text{subject to }  \eqref{Eqn_relaxed_dynamics_refined} \mbox{ and } \eqref{Eqn_y_dynamic_compact},   \mbox{ with  } x_\bsig(0)= y_\bsig(0)=x_0.
\label{Eqn_final_problem_compact}
\end{eqnarray} 
If further the above  admits  a solution  $\u^*$  among\footnote{Recall Lemma \ref{lemma_space_compact} and Corollary \ref{Corollary}  only provides $\epsilon$-optimality of controls among $\U$.}  pure controls $\U$, then  $\u^*$ is also a solution of the corresponding `pure-control problem':
\begin{eqnarray}
v_p := \sup_{\u \in \U} W(\x_\u,  \y_\u; \u) \quad \text{subject to }  \eqref{Eqn_relaxed_dynamics_refined} \mbox{ and } \eqref{Eqn_y_dynamic_compact},   \mbox{ with  } x_\u(0)= y_\u(0)=x_0,
\label{Eqn_vp_without_smooth}
\end{eqnarray}
and hence that of 
\eqref{Eqn_combined_problem}-\eqref{Eqn_x_pure_traj}---now one can   use the standard   techniques to  solve \eqref{Eqn_vp_without_smooth} and thereby compute~$\u^*$, which is also a solution of \eqref{Eqn_combined_problem}-\eqref{Eqn_x_pure_traj}.  
 

However,  the said assumption of existence of good solution 
for \eqref{Eqn_y_dynamic_compact} (and further existence of optimal among $\U$) may not be true in general. 
Although the max-trajectory~$\y$ in~\eqref{Eqn_y_defn}  exists for any admissible control   $\bsig \in \Sscr$, due to the well-posedness of the $\x$-dynamics, it is generally non-smooth (may not be differentiable)---see the discontinuity in   the right-hand side  of the corresponding ODE~\eqref{Eqn_y_dynamic_compact}. In particular, indicator  $\mathds{1}_{\{L_{mx}(s,x_\bsig (s))\ge y_\bsig (s)\}}$ induces a state-dependent discontinuity, making the direct analysis  of the control problem in \eqref{Eqn_final_problem_compact} significantly more involved---such analysis typically requires handling of Filippov   solutions, defined via differential inclusions (see e.g., \cite{barles2013bellman, filippov2013differential, rao2013hamilton}).
Rather, we replace the ODE \eqref{Eqn_y_dynamic_compact} with a `smooth approximation version' and show that the solutions of the resulting smooth-control problems provide approximate solutions to the original problem \eqref{Eqn_combined_problem}-\eqref{Eqn_x_pure_traj}.
In \cite{dhiman2024optimal}, we studied a class of  control problems, and we now show that their solutions approximate the current problem \eqref{Eqn_combined_problem}-\eqref{Eqn_x_pure_traj}. In the immediate next, we in fact propose   a more general class of smooth   problems that can approximate. %\eqref{Eqn_y_dynamic_compact}.
%that includes those in \cite{dhiman2024optimal}.



  

\subsection{The smooth control problems}
\label{subsec_smooth_approx}
The idea  is to smooth the max-trajectory~\eqref{Eqn_y_defn} by 
replacing  indicator $\mathds{1}_{\{L_{mx}(s,x_\bsig(s))\ge y_\bsig(s) \}}$  in \eqref{Eqn_y_dynamic_compact} with a  continuous  $\psi_\delta$, yielding
\begin{eqnarray}
\bdot{y}_\bsig^\delta(s) &=& \bigg ( \Delta_{mx} (s, x_\bsig (s),\sigma(s) )  \bigg  )^+  \psi_\delta(L_{mx} (s,x_\bsig(s))-y_\bsig^\delta (s))  , \mbox{ where }\label{eq:ydelta} \\
\psi_\delta(d) &:=& \phi \left(1 + \frac{d}{\delta}\right)\mathds{1}_{\{d \in [-\delta,0]\}} + \mathds{1}_{\{d>0\}}, \nonumber
\end{eqnarray}
 \begin{wrapfigure}{r}{0.33\textwidth}
\begin{center}
\vspace{-16mm}
\includegraphics[trim = {0.5cm 14.0cm 1.5cm 1.6cm}, clip, width=4.5cm, height=4.1cm]{smooth_traj.pdf}
 \vspace{-3mm}
\caption{$L_{mx}, \y_\bsig, \y_\bsig^\delta $ trajectories}
\label{Fig_y_delta}
\vspace{-5.mm}
\end{center}
\end{wrapfigure}
using  \textit{any Lipschitz continuous increasing function $\phi: [0,1] \to [0,1]$  satisfying, $\phi(0) =0$ and $\phi(1) =~1$.} 
This approximation (e.g., \cite{fleming2006controlled}) ensures Lipschitz continuity of the $\y$-ODE for any $\delta>0$, provided $\Delta_{mx}$ is sufficiently smooth, thereby enabling tractable analysis of the associated control problem. 
% \begin{figure*}[h]
% \centering
%     \begin{minipage}{5cm}
% \includegraphics[trim = {1.15cm 11.0cm 0cm 1.6cm}, clip, width=4.5cm, height=3.0cm]{y_delta.pdf}
% \end{minipage}
% \hspace{0.1cm}
%         \begin{minipage}{5cm}
% \includegraphics[trim = {0.85cm 11.0cm 0cm 1.6cm}, clip, width=4.5cm, height=3.0cm]{y_zoom.pdf}
% \end{minipage}
% \caption{Smooth (or $\y^\delta_\bsig$ in red) and non-smooth (or $\y_\bsig$ in blue) trajectories. Right figure is the expanded version of the left one  around some point of discontinuities in $\y_\bsig$. }
% \end{figure*}
Now, we propose the   smooth problems  parametrized by $\delta > 0$, which can `approximate' ($W$ is defined in \eqref{eqn_obj_fun_with_y}): 
\begin{eqnarray}
\hspace{4mm}\vr^\delta = \sup_{\bsig \in \Sscr} W(\x_\bsig,  \y_\bsig^\delta; \bsig) \quad \text{subject to }  \eqref{Eqn_relaxed_dynamics_refined} \mbox{ and } \eqref{eq:ydelta}, \mbox{ with } y_\bsig^\delta(0) = x_\bsig(0)=x_0, 
\label{Eqn_final_problem_compact_relaxed}
\end{eqnarray}
and consider  the following  extra assumptions:
\begin{enumerate} [label=\textbf{A.\arabic*}, ref=\textbf{A.\arabic*}]
\setcounter{enumi}{2}
\item  \textit{The function $L_{mx}$ is continuously differentiable. Further, there exists $K_\Delta >0$, such that for all $(s, u) \in T \times  U$ 
\begin{eqnarray*}
    | \Delta_{mx} (s, x, u ) - \Delta_{mx} (s, x', u )| &\le& K_\Delta|x-x'|,  \mbox{ for all } x, x' \in \mathbb{R}^n, \mbox{ and  } \\
    |\Delta_{mx} (s, x, u )| &\le& K_\Delta (1+ |x|), \mbox{ for all } x \in \mathbb{R}^n. 
\end{eqnarray*}
\label{assum_a3}
}
    \item \textit{$f(s, x, U):= \{f(s, x, u): u \in  U \}$ is a convex set, for each $(s, x) \in T \times \mathbb{R}^n$. }\label{assum_a4} 
%    \end{enumerate}
%\begin{enumerate} [label=\textbf{A.\arabic*}, ref=\textbf{A.\arabic*}]
%\setcounter{enumi}{4}
    \item \textit{There exists $K_r >0$, such that for all $(s, u) \in T \times  U$ 
\begin{eqnarray*}
    | L_r (s, x, u ) - L_r (s, x', u )| &\le& K_r|x-x'|,  \mbox{ for all } x, x' \in \mathbb{R}^n, \mbox{ and  } \\
    |L_r (s, x, u )| &\le& K_r (1+ |x|), \mbox{ for all } x \in \mathbb{R}^n. 
\end{eqnarray*}}
\label{assum_a5}
\end{enumerate}
We first prove that a pure control in $\U$ optimizes the smooth  problem:
\begin{lem}
\label{Lem_exist_optimal_control}
Fix any $\delta > 0$. Assume \ref{assum_a0}-\ref{assum_a3}. 

(i)  The joint ODE 
\eqref{Eqn_relaxed_dynamics_refined}-\eqref{eq:ydelta} related to problem \eqref{Eqn_final_problem_compact_relaxed}  has unique solution,  represented by   relaxed trajectories $(\x_\bsig, \y^\delta_\bsig)$, for any  $(\bsig, \delta)$. Further, 
$
\| (\x_{\bsig_n}, \y_{\bsig_n}^\delta) - (\x_{\bsig}, \y_{\bsig}^\delta) \|_\infty \to 0,$ for any sequence,  $\bsig_n \rwc \bsig$.

(ii) Additionally assume \ref{assum_a4}-\ref{assum_a5}. Then there exists an optimal solution $\u^*_\delta \in \U$, i.e., among pure controls,  for the relaxed control problem \eqref{Eqn_final_problem_compact_relaxed}.  
\end{lem}
\textbf{Proof:}  We   prove the existence of unique solution for joint ODE \eqref{Eqn_relaxed_dynamics_refined}-\eqref{eq:ydelta} and 
establish  the   continuity result of part (i), simultaneously       using Theorem \ref{thm:relaxed_controls_refined}.(b). 
Towards this, it suffices to show that the joint ODE \eqref{Eqn_relaxed_dynamics_refined}-\eqref{eq:ydelta} also satisfies the assumptions 
\ref{assum_a0}-\ref{assum_a1} required by the theorem. 
%
%The  theorem   is applicable to any relaxed trajectory given only by \eqref{Eqn_relaxed_dynamics_refined}, which satisfies \ref{assum_a0}-\ref{assum_a1}---we now show that joint trajectories of the joint ODE \eqref{Eqn_relaxed_dynamics_refined}-\eqref{eq:ydelta} also satisfy the assumptions together towards applying the same result.  The relaxed joint trajectories $(\x_\bsig, \y_\bsig^\delta)$  defined in \eqref{Eqn_relaxed_dynamics_refined}-\eqref{eq:ydelta}  are similar in structure to that in \eqref{Eqn_relaxed_dynamics_refined}, suffices to establish the required assumptions. 
The  
$\x_\bsig$ components already satisfy the required conditions by \ref{assum_a1}
and hence Theorem \ref{thm:relaxed_controls_refined}.(b) is applicable to joint $(\x_\bsig, \y_\bsig^\delta)$, if we show that the RHS of the  $\y_\bsig^\delta$-ODE in \eqref{eq:ydelta} also satisfies the Lipschitz continuity and uniform boundedness conditions of \ref{assum_a1}. These conditions  are  proved in Appendix \ref{app_lemma_exitence}. We also have  the proof of   part (ii), which is established   using the existence (among pure controls) results of \cite{roxin1962existence},  denseness of Lemma~\ref{lemma_space_compact} and the  continuity of the mapping  $\bsig \mapsto W(\x_\bsig, \y_\bsig^\delta; \bsig)$,  provided by  Theorem \ref{Thm_existence_relx_cont} and part~(i).  \eop

Thus, for smooth problems \eqref{Eqn_final_problem_compact_relaxed}, relaxed and pure controls yield the same value.
  Consequently, one may restrict the attention to   pure controls among  $\U$ and 
 the  standard numerical techniques can   compute $\u^*_\delta \in \U$, for any $\delta > 0.$


 
\subsection{Convergence}
We now move towards one of the main results of this paper, where we establish that the solution $\u^*_\delta$ of the smooth problem \eqref{Eqn_final_problem_compact_relaxed},  will  be $\epsilon$-optimal for the original problem \eqref{Eqn_combined_problem}-\eqref{Eqn_x_pure_traj}---and then any numerical solution of the smooth control problem  will be an  approximate solution for \eqref{Eqn_combined_problem}-\eqref{Eqn_x_pure_traj}, where the required level of accuracy can be derived by choosing appropriate $\delta$. 
%We discuss  the  numerical methods a little later, while the immediate attention is towards establishing  the  convergence  or the $\epsilon$-optimality result.  

The proof relies on the parametric continuity of the value function of appropriate sequence of  `control problems'   using the Maximum Theorem (see \cite[Chapter VI]{berge1877topological}). 
This theorem holds  under sufficiently general assumptions---it requires that the objective function is jointly continuous in the variable and the parameter,  and  that the domains,   one for each parameter, are sufficiently `well behaved'. 
To apply the theorem and establish the desired convergence, we first identify the objective function, parameter, and domains connecting the relaxed problems in \eqref{Eqn_combined_problem_relaxed} and \eqref{Eqn_final_problem_compact_relaxed}. We then relate their counterparts under pure controls $\U$, ultimately obtaining an approximate solution to \eqref{Eqn_combined_problem}-\eqref{Eqn_x_pure_traj}. 

We begin with the description of a  parametrized objective function that incorporates  the above   mentioned connection---consider the objective  function $\Gamma : \Sscr \times [0, \infty) \to \mathbb{R}$,    constructed using function $W$ of \eqref{eqn_obj_fun_with_y} and the parameter $\delta \ge 0$ as below: 
\begin{eqnarray}
\Gamma^* (\delta) &=& \sup_{\bsig \in \Sscr}  \Gamma  ( \bsig, \delta), \mbox{ where, }  \label{Eqn_Gamma_star}\\
    \hspace{5mm}\Gamma  ( \bsig, \delta) &:=&   W(\x_\bsig, \y_\bsig^\delta; \bsig)= \int_{0}^{t_1} L_r(t, x_\bsig(t), \sigma (t))dt  + \Psi(x_\bsig(t_1)) - y_\bsig^\delta (t_1), \mbox{ with,  } \label{Eqn_Gamma}\\
    \x_\bsig && \mbox{   the solution of the ODE \eqref{Eqn_relaxed_dynamics_refined},  and  } \nonumber\\
    \y^\delta_\bsig  &=& 
    \left \{ \begin{array}{llll}
    \mbox{  the solution of the  ODE \eqref{eq:ydelta} }      & \mbox{ when } \delta > 0,   \nonumber\\
  \mbox{ is the max-trajectory \eqref{Eqn_y_defn} }   & \mbox{ when } \delta = 0.    & 
    \end{array}
    \right . \nonumber
\end{eqnarray}
In the above,   any relaxed control $\bsig \in \Sscr$ forms a decision variable and the parameter $\delta $ links the required optimization problems,   because of the following reasons:
\begin{itemize}
    \item    the optimization problem  $ \sup_{\bsig\in \Sscr}\Gamma  ( \bsig, \delta) $, for any $\delta > 0$, exactly equals the smooth-problem  \eqref{Eqn_final_problem_compact_relaxed}, in other words,   $\vr^\delta =  \Gamma^*  (   \delta) $;  
    \item 
    for $\delta=0$, $\sup_{\bsig\in\Sscr}\Gamma(\bsig,\delta)$ is the original relaxed problem in \eqref{Eqn_combined_problem_relaxed}, so $\Gamma^*(0)$ equals its value.
\end{itemize}
Thus, the idea behind establishing the desired convergence (and then $\epsilon$-optimality) is to show that the  value function $\Gamma^*(\delta)$ is continuous wrt $\delta$. 
More precisely, we only require the continuity at $\delta = 0$, i.e., 
  the convergence of the relaxed values, 
\(
\Gamma^*(\delta_n) \to \Gamma^*(0), 
\)
for  any given sequence $\delta_n \stackrel{n \to \infty}{ \longrightarrow} 0$; let $\Theta := \{\delta_n\}_{n\ge 1}$.
To this end, 
we  apply  the  Maximum Theorem to  the parametrized function $\Gamma$ defined in \eqref{Eqn_Gamma}, after  restricting its joint domain to  $\Sscr \times \Theta$, by   proving  the following major steps:

\begin{enumerate}[label=(\textbf{\Roman*}), ref=(\textbf{\Roman*})]
\setcounter{enumi}{0}
\item  let $\Sscr_\delta$ represent the domain of optimization, when the parameter is $\delta$, then one needs to prove that $\delta \mapsto \Sscr_\delta$ is compact and continuous correspondence.  \label{step_I}
\item  one needs to prove that $\Gamma$ is jointly continuous at  $(\bsig, \delta) \in \Sscr\times \Theta$ in some appropriate topology. 
\label{step_II}
\end{enumerate} 

First, observe that the domain of optimization is the same  for any  $\delta$, i.e.,   
    $\Sscr_\delta = \Sscr$
    and thus the Step  \ref{step_I} is immediate by   
 Lemma \ref{lemma_space_compact}, after  empowering $\Sscr$ with r-weak  topology.  
 
 Towards proving the Step  \ref{step_II},   it suffices to  establish sequential continuity, as $\Sscr$ is metrizable by Lemma \ref{lemma_space_compact}.
%
By Theorems \ref{thm:relaxed_controls_refined}-\ref{Thm_existence_relx_cont}, we have already proved that 
the  trajectory $\x_\bsig$, the  max trajectory $\y_\bsig = \y^{0}_\bsig$ and the running cost $L_r$ are sequentially continuous wrt the relaxed control $\bsig$. Further  $\x_\bsig$ and $L_r$  do not depend upon $\delta$.  
\newcommand{\II}{{\mathbb I}}
We next \textit{establish the joint continuity of the max-trajectory $\y_\bsig^\delta$ wrt   $(\bsig, \delta) \in \Sscr \times \Theta$}:
\begin{thm}[{\bf $(\bsig,\delta)$-continuity}] 
\label{Thm_ydel_convg} Assume \ref{assum_a0}-\ref{assum_a3}. 
 Then  $\{\y^0_\bsig: \bsig \in \Sscr\}$, the  max-trajectories of \eqref{Eqn_y_defn},  and $\{(\x_\bsig, \y^\delta_\bsig):  \bsig\in \Sscr, \delta > 0\}$,  the solutions   of  \eqref{Eqn_relaxed_dynamics_refined}-\eqref{eq:ydelta}   satisfy
the following continuity results   in uniform topology. 

(i)  Fix $\delta> 0$.  
Then 
$
\| (\x_{\bsig_n}, \y_{\bsig_n}^\delta) - (\x_{\bsig}, \y_{\bsig}^\delta) \|_\infty \to 0,$ for any sequence,  $\bsig_n \rwc \bsig$.

(ii) Fix $\bsig \in \Sscr$ and  $\delta > 0$. Then 
$\|\y^{\delta}_\bsig -  \y^0_\bsig \|_\infty \le \delta$. 
%and hence  $\|\y^{\delta}_\bsig -  \y^0_\bsig \|_\infty \to 0,$   for any sequence $\delta_n \to  0$. 

  (iii) Further,  
$
\| (\x_{\bsig_n}, \y_{\bsig_n}^{\delta_n}) - (\x_{\bsig}, \y_{\bsig}^0) \|_\infty \to 0,$ for any    $\bsig_n \rwc \bsig$ and $\delta_n \to 0$.


\end{thm}
\textbf{Proof:} \textbf{Part (i)} is directly given by part (i) of Lemma \ref{Lem_exist_optimal_control}. \\
\textbf{Part (ii):}
We first define the following brief notations and some definitions:
 $$L_{mx}(t) = L_{mx}(t, x(t)), \  \  \bdot{L}_{mx} (t) = \Delta_{mx} (t, x(t), u(t) ), \mbox{ for any }  t. 
 $$  
Define $\Dw_0  := 0,$ and then the  following terms  for each  $i \ge 1$, recursively using \eqref{eq:ydelta},  
\begin{eqnarray}
    && \hspace{14mm}\Up_i := \inf\{ t > \Dw_{i-1}: L_{mx}(t)> y^\delta(t) - \delta, \ \bdot{L}_{mx}(t) >0 \} = \inf\{ t > \Dw_{i-1}:  \bdot{y}^\delta(t)  >0 \}, \nonumber\\
   && \hspace{14mm} \Dw_i := \inf\{ t > \Up_i: L_{mx}(t) \le  y^\delta(t) - \delta \mbox{ or }  \bdot{L}_{mx}(t) \le  0 \}=  \inf\{ t > \Up_i:  \bdot{y}^\delta(t)  =0 \} \label{Eqn_definition_ui_di}
\end{eqnarray}
(we suppress $\bsig$ while retaining $\delta$ in notations for simplicity and clarity). 
Continue the above definitions till one of them touches $t_1$ and  
these imply the following:
 $$
 \bdot{y}^\delta(t)  =0  \mbox{ for any } t \in \cup_{i\ge 1} [ \Dw_{i-1}, \Up_i], \mbox{ while,  } \bdot{y}^\delta(t)  > 0  \mbox{ for any } t \in \cup_{i\ge 1} [  \Up_i, \Dw_{i}]. 
 $$
Towards proving part (ii), it   suffices to prove the following,
\begin{eqnarray}
&&y^0(t) \le     y^\delta (t) \le y^0 (t) + \delta,  \mbox{ for all } t \in T. 
\label{Eqn_Sw}
\end{eqnarray}
As the functions involved in \eqref{Eqn_definition_ui_di} are absolutely continuous,  one can have at most countably many  $\{\Dw_i, \Up_i\}_i$ (see \cite{royden2010real}).
Thus, the result is derived using
 mathematical induction on $i$: with  $\II_\ell := (\Up_\ell, \Dw_\ell) \cup [\Dw_\ell, \Up_{\ell+1}]$ for each $\ell$,  we prove \eqref{Eqn_Sw}     for all $t \in   \II_i$,  assuming the  same for  all previous intervals, i.e., for all $t \in \cup_{\ell < i} \II_\ell$. Detailed proof is in  Appendix \ref{app_thm_y_ctny}. 


\textbf{Part (iii):} For the given pair of sequences, one can split using   triangle inequality  as below and then using the upper bound of part (ii), which is uniform across $\bsig \in \Sscr$:
\begin{eqnarray*}
\|(\x_{\bsig_n}, \y^{\delta_n}_{\bsig_n}) - (\x_{\bsig}, \y^0_{\bsig})\|_\infty
 &\le &  \|(\x_{\bsig_n},\y^{\delta_n}_{\bsig_n})- (\x_{\bsig_n},\y^{0}_{\bsig_n}
    )\|_\infty 
    + \|(\x_{\bsig_n},\y^{0}_{\bsig_n}) - (\x_{\bsig}, \y^0_{\bsig})\|_\infty \\
    &\le & \delta_n  + \|(\x_{\bsig_n}, \y^{0}_{\bsig_n}) - (\x_{\bsig}, \y^0_{\bsig})\|_\infty. 
 \end{eqnarray*}
Next, the above converges to $0$ as $n \to \infty$ using Theorem \ref{thm:relaxed_controls_refined}.(b) and Theorem \ref{Thm_existence_relx_cont}.(a).(ii). \eop

Thus, we have established the  continuity arguments of various components that build  the  objective function $\Gamma$. 
We finally establish the major result of this paper:
\begin{thm} [{\bf Approximation and  convergence}] 
\label{Thm_epsilon_optimality}Assume \ref{assum_a0}-\ref{assum_a5} and  
consider    $\delta_n \to 0.$   
Then with $\u_n^*$ representing the solution of Lemma \ref{Lem_exist_optimal_control},  for each  $n$, we have:
$$
\lim_{n \to \infty}
\left |  \Gamma (\u^*_n, 0)  - \Gamma^* (0) \right | = 0, \mbox{ where  }
\Gamma (\u^*_n, 0) = J(x_0; \u_n^*), 
$$%
is the objective function of  \eqref{Eqn_combined_problem}    and $\Gamma^* (0)$ is the corresponding value. 
\end{thm}
\textbf{Proof:} 
Consider  any arbitrary sequence $\{\bsig_n\}_{n \geq 1}  \subset \Sscr$ such that $\bsig_n \rwc \bsig \in \Sscr$.  
Then,
\begin{eqnarray*}
  \Gamma(\bsig_n, \delta_n) &=&   \int_{0}^{t_1} L_r(t, x_{\bsig_n} (t), \sigma_n (t))dt  - y_{\bsig_n}^{\delta_n} (t_1) + \Psi(x_{\bsig_n}(t_1)) \\
  && \hspace{-3mm} \to \  \int_{0}^{t_1} L_r(t, x_\bsig (t), \sigma (t))dt  \  \  - y_{\bsig}^{0} (t_1) + \Psi(x_{\bsig}(t_1))=  \Gamma(\bsig,  0),
\end{eqnarray*}
establishing  sequential continuity of $\Gamma$ on $\Sscr\times \Theta$, with $\Theta = \{\delta_n\}$, 
because of the following:\\
%steps:
$\bullet$ integral terms converge by Theorem \ref{Thm_existence_relx_cont}.(a).(i), observe initial condition $x_0$ is fixed;\\
$\bullet$ second and third   terms converge 
     by Theorem \ref{Thm_ydel_convg}.(iii) and continuity of $\Psi$ (by \ref{assum_a2}).

Thus,  the Maximum Theorem (see \cite[Chapter VI]{berge1877topological}) is applicable  (see also Step \ref{step_I}) and hence we have:  $\Gamma^*(\delta_n) \to \Gamma^*(0).$
Also, by Lemma \ref{Lem_exist_optimal_control},   $\Gamma^*(\delta_n) = \Gamma( \u_n^*, \delta_n)$, for any $n$.    Thus,  
from \eqref{Eqn_Gamma} and by uniform (across   $\bsig$ or $\u$) upper bound of  Theorem \ref{Thm_ydel_convg}.(ii), we have, 
 \begin{eqnarray*}
 \left |  \Gamma (\u_n^*,  0)  - \Gamma^* (0) \right | &\le&   \left |  \Gamma (\u_n^*,  0) - \Gamma(\u_n^*, \delta_n)  \right | + \left |  \Gamma (\u_n^*,  \delta_n) - \Gamma^*(0)  \right | \\
&& \hspace{-10mm} =\ |y^{\delta_n}_{\u_n^*} (t_1) - y^{0}_{\u_n^*} (t_1) |  + \left |  \Gamma^* (  \delta_n) - \Gamma^*(0)  \right | \ 
\le  \delta_n  + \left |  \Gamma^* (  \delta_n) - \Gamma^*(0)  \right | \to  0. \  \mbox{ \eop }
 \end{eqnarray*}
    


\ignore{
Finally, our aim is to show that for every $\epsilon>0$, there exists a $\delta_\epsilon>0$, such that 
$|J(x_0;\u_\delta^*,0) - \Gamma^*(0)| 
\le \epsilon, 
\mbox{ for all } \delta \le \delta_\epsilon. $
Towards this, we split the term like 
\begin{eqnarray}
|J(x_0;\u_\delta^*,0) - \Gamma^*(0)| 
&\le& |J(x_0;\u_\delta^*,0) - J(x_0;\u_\delta^*,\delta)|  + |J(x_0;\u_\delta^*,\delta) - \Gamma^*(0)|,  
\label{Eqn_thm4_final_ineq}
\end{eqnarray}
and show that both the quantities on RHS are less than $\nicefrac{\epsilon}{2}$. 

First we consider the second term $|J(x_0;\u_\delta^*,\delta) - \Gamma^*(0)|$. 
Using the continuity of $\Gamma^*(\delta)$  at $\delta = 0$ from \eqref{Eqn_Gamma_Star_converg}, we have that for every $\epsilon > 0$, there exists $\delta_1 > 0$ such that for all $\delta \leq \delta_1$,
$|\Gamma^*(\delta) - \Gamma^*(0)| \leq \nicefrac{\epsilon}{2}$. 
%This means that for sufficiently small $\delta$, the optimal value of the approximate problem is close to that of the original problem. 
Using \eqref{Eqn_J_ustar_equal_Gam_star}, we have 
\begin{equation}
 |J(x_0;\u_\delta^*,\delta)- \Gamma^*(0)| \le \nicefrac{\epsilon}{2}, \mbox{ for all } \delta \le \delta_1. 
 \label{Eqn_thm4_first_ineq}
\end{equation}

Next, we  consider the first term in RHS of \eqref{Eqn_thm4_final_ineq}, i.e., $|J(x_0;\u_\delta^*,0) - J(x_0;\u_\delta^*,\delta)|$. Observe that for a fixed control $\u_\delta^*$, the  state trajectory $\x$ and the running cost $L_r$ are independent of $\delta$ and hence continuous wrt $\delta$. By Theorem \ref{Thm_ydel_convg}.(i), $\y$ is  continuous in $\delta$ (observe that $\U \subset \Sscr$). Thus overall,  using the continuity of the integrand and standard convergence arguments, we obtain
$
J(x_0;\u_\delta^*,\delta) \to J(x_0;\u_\delta^*,0), \text{ as } \delta \to 0.$
Therefore, for every $\epsilon > 0$, there exists $\delta_2 > 0$ such that for all $\delta \le \delta_2$,
\begin{eqnarray}
    |J(x_0;\u_\delta^*,0) - J(x_0;\u_\delta^*,\delta)| \le \nicefrac{\epsilon}{2}.
     \label{Eqn_thm4_second_ineq}
\end{eqnarray}
Using \eqref{Eqn_thm4_final_ineq}-\eqref{Eqn_thm4_second_ineq}, for $\delta \le \delta_\epsilon= \min\{\delta_1,\delta_2\}$, we obtain
$|J(x_0;\u_\delta^*,0) - \Gamma^*(0)| 
\le  \nicefrac{\epsilon}{2} + \nicefrac{\epsilon}{2}= \epsilon.$




Observe that $ \Gamma^*(0) $ and  $ J(x_0;\u_\delta^*,0) $ represents the optimal value $\vr$ and $\vp$ of control problems \eqref{Eqn_combined_problem_relaxed} and \eqref{Eqn_combined_problem} respectively. 
Hence, the control $\u_\delta^*$ achieves a cost arbitrarily close to the optimal value of the original problem \eqref{Eqn_combined_problem}. Therefore, $\u_\delta^*$ is $\epsilon$-optimal for \eqref{Eqn_combined_problem}.} 



\ignore{
\newpage

Towards this, first observe that the control space $\Sscr$ is compact under the r-weak topology by Lemma \ref{lemma_space_compact}. And thus, we now shift the original control problem \eqref{Eqn_combined_problem} to relaxed control problem \eqref{Eqn_relaxed_dynamics_refined}--\eqref{Eqn_combined_problem_relaxed}. Then, observe that the admissible control set for both the original relaxed problem \eqref{Eqn_relaxed_dynamics_refined}--\eqref{Eqn_combined_problem_relaxed} and its smooth approximation $\Prb_p^\delta$ coincide with the same set $\Sscr$. Hence, the feasible correspondence $\delta \mapsto \Sscr$ is constant (independent of $\delta$), and therefore trivially continuous and compact-valued.

 Under assumptions \ref{assum_a0}-\ref{assum_a4}, using  \cite[Theorem 1]{dhiman2024optimal}, there exists an optimal control (say $\u_\delta^*$) for  problem \eqref{Eqn_final_problem_compact}. 
By Lemma \ref{lemma_space_compact}, $\U$ is dense in  $\Sscr$---for every $\epsilon>0$, there exists $\u_\epsilon \in \U$, such that for every $\delta>0$, 
$J(x_0; \u_\epsilon, \delta) \le \vr(\delta) + \epsilon$.  Also, $\U \subset \Sscr$, thus $\vr(\delta) \le J(x_0; \u_\epsilon^*, \delta)$. Overall, we have 
$$
\vr(\delta) \le J(x_0; \u_\epsilon^*, \delta) \le J(x_0; \u_\epsilon, \delta) \le \vr(\delta) + \epsilon. 
$$
As $\epsilon>0$ is arbitrary, consider $\epsilon \to 0$, we get $\vr(\delta) = J(x_0; \u_\epsilon^*, \delta)$. 
Thus, we consider the same compact set $\Sscr$ for both original and relaxed control. 



Define the  objective functional $\Gamma : \Sscr \times \mathbb{R}_+ \to \mathbb{R}$ is defined over the space of relaxed controls $\Sscr$  and with $\delta \in \mathbb{R}_+ $  that connects the  problems $\Prb_r^\delta$ with $\delta > 0$ given in \eqref{Eqn_final_problem_compact} to the one without smooth approximation  \eqref{Eqn_relaxed_dynamics_refined}-\eqref{Eqn_combined_problem_relaxed} (which we index by $\delta= 0$) by considering a combined objective function as below:
\begin{eqnarray*}
    \Gamma (x_0; \bsig, \delta) &:=&   \int_{0}^{t_1} L_r(t, x^\delta_\bsig(t), \sigma (t))dt  + \Psi(x^\delta_\bsig(t_1)) - y_\bsig^\delta (t_1), \mbox{ where } \\
    \y^\delta_\sigma  &=& 
    \left \{ \begin{array}{llll}
    \mbox{ is solution of ODE \eqref{Eqn_final_problem_compact_relaxed} }      & \mbox{ when } \delta > 0,   \\
  \mbox{ is the max-trajectory \eqref{Eqn_y_defn} }   & \mbox{ when } \delta = 0.   & 
    \end{array}
    \right .
\end{eqnarray*}

We now establish that the objective functional $\Gamma(x_0;\bsig,\delta)$ is jointly continuous in $(\bsig,\delta)$. From Theorem \ref{Thm_existence_relx_cont}, the  max trajectory $\y_\bsig$ and the running cost $L_r$ are continuous wrt the relaxed control $\bsig$ and the initial condition $x_0$. Therefore, \textit{it suffices to establish continuity of the max-trajectory $\y_\bsig$ wrt the smoothing parameter $\delta$}. Once this is shown, it follows that the entire objective functional, which depends on $\y_\bsig$ and $L_r$, is jointly continuous in $(\bsig,\delta)$. There are three cases possible:
\begin{itemize}
    \item There is a sequence $\delta_n$, such that $\delta_n =0$, for all $n$, then we know that $\delta_n \to 0$. This implies that $\y_\bsig^{\delta_n}$ is max-trajectory \eqref{Eqn_y_defn} for all $n$. And thus, the $\y_\bsig^{0}$ is also the same \eqref{Eqn_y_defn}. 
    \item The same arguments follows for the sequence $\delta_n \to \delta$, where both $\delta_n>0$ and $\delta>0$. As here the corresponding  $\y$ trajectories are solution of \eqref{Eqn_final_problem_compact_relaxed}. 
    \item Consider the sequence $\delta_n \to \delta$, where $\delta_n >0$, for all $n$ and $\delta =0$. The continuity of $\y$ in this case is established immediately below in Theorem \ref{Thm_ydel_convg}. 
\end{itemize}

Having verified the conditions of the Maximum Theorem, we conclude that the corresponding value function
$\vr(\delta) := \inf_{\bsig \in \Sscr} \Gamma(x_0;\bsig,\delta)$ 
is continuous in the parameter $\delta$.
In particular, 
$\vr(\delta_n) \to \vr(\delta)$ as $\delta_n \to \delta$, 
where $\vr(0)$ corresponds to the value of the control problem \eqref{Eqn_relaxed_dynamics_refined}-\eqref{Eqn_combined_problem_relaxed}.

% We now outline the key steps required for applying the Maximum Theorem:

% \medskip

% \noindent
% {\bf Step 1: Compactness and continuity of the feasible correspondence.}
% By Lemma \ref{lemma_space_compact}, the control space $\Sscr$ is compact under the r-weak topology. Furthermore, observe that the admissible control set for both the original relaxed problem \eqref{Eqn_relaxed_dynamics_refined}--\eqref{Eqn_combined_problem_relaxed} and its smooth approximation $\Prb_p^\delta$ coincide with the same set $\Sscr$. Hence, the feasible correspondence is constant (independent of $\delta$), and therefore trivially continuous and compact-valued.

% \medskip

% \noindent
% {\bf Step 2: Joint continuity of the objective functional.}
% We now establish that the objective functional $J(x_0;\bsig,\delta)$ is jointly continuous in $(\bsig,\delta)$. From Theorem \ref{Thm_existence_relx_cont}, the  max trajectory $\y_\bsig$ and the running cost $L_r$ are continuous with respect to the relaxed control $\bsig$ and the initial condition $x_0$. Therefore, \textit{it suffices to establish continuity of the max-trajectory $\y_\bsig$ with respect to the smoothing parameter $\delta$}. Once this is shown, it follows that the entire objective functional, which depends on $\y_\bsig$ and $L_r$, is jointly continuous in $(\bsig,\delta)$.


% \medskip


% \noindent
% {\bf Step 3: Maximum Theorem and Convergence.}
% Having verified the conditions of the Maximum Theorem, we conclude that the corresponding value function
% $\vr(\delta) := \inf_{\bsig \in \Sscr} J(x_0;\bsig,\delta)$ 
% is continuous in the parameter $\delta$. In particular, 
% $\vr(\delta) \to \vr(0)$ as $\delta \to 0$, 
% where $\vr(0)$ corresponds to the value of the control problem \eqref{Eqn_relaxed_dynamics_refined}-\eqref{Eqn_combined_problem_relaxed}. Moreover, any sequence of optimal controls ${\bsig_\delta^*}$ associated with the problems $\Prb_p^\delta$ has a convergent subsequence (in the r-weak topology) whose limit is an optimal control for the problem \eqref{Eqn_relaxed_dynamics_refined}-\eqref{Eqn_combined_problem_relaxed}.
% % This establishes consistency of the smooth approximation at the level of both value functions and optimal controls.



To complete the argument, it remains to establish the continuity of the max-trajectory $\y_\bsig$ with respect to $\delta$. Towards this, for a fixed relaxed control $\bsig \in \Sscr$, we now proceed to analyze the dependence of $\y_\bsig$ on the smoothing parameter $\delta$.



\begin{thm}
    Assume \ref{assum_a0}-\ref{assum_a1}. Then $v_{\bsig_n}(\delta_n) \to v_\bsig \ \text{as } \delta_n \to 0.$ and $\bsig_n \rwc \bsig$. 
\end{thm}
\textbf{Proof:} Using the continuity of $\y$ wrt relaxed controls $\bsig$ and  $\bsig_n \rwc \bsig$, it follows that for any fixed $\delta_n$, the corresponding trajectories satisfy $\|y^{\delta_n}_{\bsig_n} - y^{\delta_n}_{\bsig}\|_\infty \to 0$ as $n \to \infty$. 


Further, by the convergence of the smooth approximation to the original trajectory, we also have $\|y^{\delta_n}_{\bsig} - y^{0}_{\bsig}\|_\infty \to 0$ as $\delta_n \to 0$. Combining these two facts and using the triangle inequality yields $\|y^{\delta_n}_{\bsig_n} - y^{0}_{\bsig}\|_\infty \le \|y^{\delta_n}_{\bsig_n} - y^{\delta_n}_{\bsig}\|_\infty + \|y^{\delta_n}_{\bsig} - y^{0}_{\bsig}\|_\infty \to 0$ as $n \to \infty$. 

Consequently, by continuity of the cost functional wrt the trajectory, we obtain $\Gamma(x_0;\bsig_n,\delta_n) \to \Gamma(x_0;\bsig,0)$. Finally, noting that the control space for both the original relaxed problem \eqref{Eqn_relaxed_dynamics_refined}--\eqref{Eqn_combined_problem_relaxed} and its smooth approximation is the same compact set $\Sscr$, the associated feasible correspondence is constant and hence continuous; therefore, using the Maximum Theorem implies convergence of the value functions, yielding $v_{\bsig_n}^{\delta_n} \to v_\bsig$ as $n \to \infty$. \eop

\begin{thm} [{\bf  $\epsilon$-optimality}] Assume \ref{assum_a0}-\ref{assum_a4}. 
    For $\epsilon>0$, there exists a $\delta_\epsilon>0$, such that $\u_\delta^*$ is $\epsilon$-optimal to the control problem \eqref{Eqn_combined_problem}, for all $\delta \le \delta_\epsilon$. 
\end{thm}
\textbf{Proof:} 
We now establish the $\epsilon$-optimality of the solution obtained from the approximate problem. Under assumptions \ref{assum_a0}-\ref{assum_a4}, using  \cite[Theorem 1]{dhiman2024optimal}, there exists an optimal control (say $\u_\delta^*$) for  problem \eqref{Eqn_final_problem_compact}. 
By Lemma \ref{lemma_space_compact}, $\U$ is dense in  $\Sscr$---for every $\epsilon>0$, there exists $\u_\epsilon \in \U$, such that for every $\delta>0$, 
$J(x_0; \u_\epsilon, \delta) \le \vr(\delta) + \epsilon$.  Also, $\U \subset \Sscr$, thus $\vr(\delta) \le J(x_0; \u_\epsilon^*, \delta)$. Overall, we have 
$$
\vr(\delta) \le J(x_0; \u_\epsilon^*, \delta) \le J(x_0; \u_\epsilon, \delta) \le \vr(\delta) + \epsilon. 
$$
As $\epsilon$ is arbitrary, take $\epsilon \to 0$, we have $\vr(\delta) = J(x_0; \u_\epsilon^*, \delta)$. 


Also, for every  $\epsilon > 0$,   there exists $\delta_\epsilon > 0$ such that for all $\delta \le \delta_\epsilon$,
$|\vr(\delta) - \vr(0)| \le \epsilon.$
Using optimality of $\u_\delta^*$ for the $\delta$-problem, it follows that
$J(x_0;\u_\delta^*,\delta) = \vr(\delta) \le \vr(0) + \epsilon.$
% Thus, the control $\u_\delta^*$ achieves a cost within $\epsilon$ of the optimal value of the original problem. 
Hence, $\u_\delta^*$ is $\epsilon$-optimal for \eqref{Eqn_combined_problem}. \eop

\begin{thm}
    Assume \ref{assum_a0}-\ref{assum_a1}. Then $v_{\bsig_n}(\delta_n) \to v_\bsig \ \text{as } \delta_n \to 0.$ and $\bsig_n \rwc \bsig$. 
\end{thm}
\textbf{Proof:} Using the continuity of $\y$ wrt relaxed controls $\bsig$ and  $\bsig_n \rwc \bsig$, it follows that for any fixed $\delta_n$, the corresponding trajectories satisfy $\|y^{\delta_n}_{\bsig_n} - y^{\delta_n}_{\bsig}\|_\infty \to 0$ as $n \to \infty$. 


Further, by the convergence of the smooth approximation to the original trajectory, we also have $\|y^{\delta_n}_{\bsig} - y^{0}_{\bsig}\|_\infty \to 0$ as $\delta_n \to 0$. Combining these two facts and using the triangle inequality yields $\|y^{\delta_n}_{\bsig_n} - y^{0}_{\bsig}\|_\infty \le \|y^{\delta_n}_{\bsig_n} - y^{\delta_n}_{\bsig}\|_\infty + \|y^{\delta_n}_{\bsig} - y^{0}_{\bsig}\|_\infty \to 0$ as $n \to \infty$. 

Consequently, by continuity of the cost functional wrt the trajectory, we obtain $J(x_0;\bsig_n,\delta_n) \to J(x_0;\bsig,0)$. Finally, noting that the control space for both the original relaxed problem \eqref{Eqn_relaxed_dynamics_refined}--\eqref{Eqn_combined_problem_relaxed} and its smooth approximation is the same compact set $\Sscr$, the associated feasible correspondence is constant and hence continuous; therefore, using the Maximum Theorem implies convergence of the value functions, yielding $v_{\bsig_n}^{\delta_n} \to v_\bsig$ as $n \to \infty$. \eop


\begin{thm} Assume \ref{assum_a0}-\ref{assum_a4}. 
    For $\epsilon>0$, there exists a $\delta_\epsilon>0$, such that $\u_\delta^*$ is $\epsilon$-optimal to the control problem \eqref{Eqn_combined_problem}, for all $\delta \le \delta_\epsilon$. 
\end{thm}
\textbf{Proof:} 
From \cite[Theorem 1]{dhiman2024optimal}, for every $\delta > 0$, there exists a control $\u_\delta^* \in \U$ such that
$$
\vp(\delta) := \inf_{\u \in \U} J(x_0;\u,\delta)
= J(x_0;\u_\delta^*,\delta).
$$

By Lemma \ref{lemma_space_compact}, the set of ordinary controls $\U$ is dense in the relaxed control space $\Sscr$. Hence, for any $\epsilon > 0$, there exists a control $\u_\epsilon \in \U$ such that
$$
J(x_0;\u_\epsilon,\delta) \le v_\bsig(\delta) + \epsilon.
$$


Since $\U \subset \Sscr$, it follows that
$$
v_\bsig(\delta) \le J(x_0;\u_\delta^*,\delta).
$$
Combining this with the definition of $\u_\delta^*$ and the approximation above, we obtain
$$
v_\bsig(\delta)
\le J(x_0;\u_\delta^*,\delta)
\le J(x_0;\u_\epsilon,\delta)
\le v_\bsig(\delta) + \epsilon.
$$
Since $\epsilon > 0$ is arbitrary, letting $\epsilon \to 0$ yields
$$
J(x_0;\u_\delta^*,\delta) = v_\bsig(\delta).
$$
Thus, $\u_\delta^*$ is optimal for the $\delta$-regularized problem \eqref{Eqn_final_problem_compact}.


By Theorem \ref{Thm_ydel_convg} and using the Maximum Theorem, the value functions satisfy
$$
v_\bsig(\delta) \to v_\bsig \quad \text{as } \delta \to 0.
$$



Let $\epsilon > 0$ be given. Since $v_\bsig(\delta) \to v_\bsig$, there exists $\delta_\epsilon > 0$ such that for all $\delta \le \delta_\epsilon$,
$$
|v_\bsig(\delta) - v_\bsig| \le \epsilon.
$$
Using optimality of $\u_\delta^*$ for the $\delta$-problem, we have
$$
J(x_0;\u_\delta^*) = v_\bsig(\delta) \le v_\bsig + \epsilon.
$$
This shows that $\u_\delta^*$ is $\epsilon$-optimal for the original control problem \eqref{Eqn_combined_problem}.
This completes the proof. \eop
}

